Characterizing LLM Abstention Behavior in Science QA with Context Perturbations

The correct model response in the face of uncertainty is to abstain from answering a question so as not to mislead the user. In this work, we study the ability of LLMs to abstain from answering context-dependent science questions when provided insufficient or incorrect context. We probe model sensitivity in several settings: removing gold context, replacing gold context with irrelevant context, and providing additional context beyond what is given. In experiments on four QA datasets with six LLMs, we show that performance varies greatly across models, across the type of context provided, and also by question type; in particular, many LLMs seem unable to abstain from answering boolean questions using standard QA prompts. Our analysis also highlights the unexpected impact of abstention performance on QA task accuracy. Counter-intuitively, in some settings, replacing gold context with irrelevant context or adding irrelevant context to gold context can improve abstention performance in a way that results in improvements in task performance. Our results imply that changes are needed in QA dataset design and evaluation to more effectively assess the correctness and downstream impacts of model abstention.

==> old/abs.tex <==
The few-shot capability of large language models (LLMs) has emerged as a powerful approach for addressing knowledge-intensive tasks like scientific question answering (QA). 
Closed-book science QA tasks provide models with informational contexts from which to answer a question, but how an LLM's parametric memory interacts with errors in provided context remains under-explored.

In this work, we investigate the impact of incorrect context on LLM performance on science QA tasks, ranging from highly context-sensitive tasks such as document-based scientific QA to less context-sensitive tasks such as factoid QA. We study model sensitivity in two settings: swapping gold context with no context or irrelevant context and providing more context on top of given context. In experiments on four QA datasets and five models, we show that model performance (especially on unanswerable questions) not only varies significantly based on the type and quantity of context provided but also is highly impacted by question types. Also the performance varies across models are huge. As a solution, we show that providing irrelevant or ambiguous context during in-context learning mitigates some of these issues.
We hope our analysis can provide insights to the community on how to handle context during training for science QA tasks.


==> old/conclusion.tex <==
\section{Conclusion}

==> old/discussion.tex <==
\section{Discussion \& Conclusion}

We study LLM response to noisy context during prompting for science QA. 
% We divide the model's uncertainty in two perspectives: prediction with abstention and distractibility. We develop a new framework by prompting LLMs using various type of context to better evaluate model's prediction with abstention and distractibility. 
We find that both ChatGPT and GPT-3 are sensitive to noisy context, though providing noisy context during ICL mitigates performance degradation.
Context sensitivity should be noted when assessing LLM performance. We hope our framework can be used to evaluate and mitigate LLM performance loss due to noisy context in future work.
% Inspired by these findings, we may adopt strategy like mixture of experts to ensemble different LLMs to solve complex tasks \lucy{what?}.

==> old/exp.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{p{13mm}p{10mm}p{9mm}p{15mm}p{8mm}}
\toprule
 Dataset & Context length & Unans. ratio & Answer types & Testset Size \\ 
\midrule 
\squad  &   128  & 0.5 & Ext & 11873\\
\pubmedqa   &  204 & 0.1 & Bool &  500\\
\qasper  & 226 & 0.1 & Ext/Abs/Bool & 1451\\
BioASQ  & 270 & 0.0 & Bool & 140\\
\bottomrule
\end{tabular}
  \caption{Dataset statistics.}
\label{tab:datasets}
\end{table}

\input{tables/answerc_change}
\input{tables/model_answerability}




\begin{figure*}[h]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/qasper_type_ans.pdf}
        \caption{\qasper}
        \label{fig:sub1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/squad2_type_ans.pdf}
        \caption{\squad}
        \label{fig:sub2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/pubmed_type_ans.pdf}
        \caption{\pubmedqa}
        \label{fig:sub3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figure/bioasq_type_ans.pdf}
        \caption{BioASQ}
        \label{fig:sub4}
    \end{subfigure}
    \caption{Results for the abstention ability of LLAMAv2 based on question types for four datasets.We could see that LLamaV2 are relunctant to abtain from boolean questions. For unanswerable questions, more context causes model to hallucinate.  }
    \label{fig:main}
\end{figure*}




% \section{Experiment}

% This section presents our experimental setup (\S\ref{sec:experimental_setup}) for the evaluation of the proposed framework concerning two aspects: prediction with abstention(§4.2) and distractibility (§4.3).

% \subsection{Experimental Setup}
% \label{sec:experimental_setup}
% Our experiments are conducted using chatGPT and text-davinci-002. We conduct experiments in two different settings: zero-shot and few-shots settings. We set the temperature as 0 and top p sampling as 1 to decrease the randomness of model output. \lucy{move models to end of section 3 and create two sections for prediction with abstention and distractibility; the current organization is too messy (with the nested results sections)}

\section{Prediction with abstention}
\label{sec:prediction_w_abstention}

We introduce the concept of context-sensitivity to estimate the extent of context-dependence of our three QA datasets given a particular model. We measure context-sensitivity by removing all context from all questions and asking models to provide answers. The proportion of questions for which the model abstains (i.e., predicts ``unanswerable'') is interpreted as the context-sensitivity of the dataset from the perspective of the given model. The intuition is that if a model tends to use parametric knowledge to answer a question without context, correctly or incorrectly, then the model does not consider the question to be context-sensitive. A dataset that has many such questions is itself considered to be less context-sensitive. 
% \lucy{what is the relationship between context-sensitivity, answerability, and prediction with abstention? not sure what i'm supposed to get out of this section with some many terms and definitions} Answerability is defined as the as accuracy for predicting the special token “unanswerable” given no context or random context. I would say these three are equal. We could just use one to unify the terms. high answerability = context-sensitivity  = prediction with abstention \lucy{+1 please combine to reduce confusion}

If a dataset is context-sensitive, then answerable questions within the dataset should become unanswerable if the context is removed. We test this by reporting the proportion of questions in each dataset for which the model responds ``unanswerable'' when no context is provided. We report results in Table~\ref{tab:noAns_f1_no_context}; HasAns are questions for which a context-dependent answer is provided in the dataset, and NoAns are questions the dataset labels as unanswerable.

PubmedQA and bioASQ are not context-dependent compared to SQUAD2 and qasper.



% , 
% we report model context-sensitivity
% \lucy{what is answerability score? Answerability is defined as the as accuracy for predicting the special token “unanswerable” given no context or random context} 
% on the questions for which a (context-dependent) answer is provided in the dataset (HasAns), and on questions for which no answer is provided in the dataset (NoAns) (i.e., the ground truth response is ``unanswerable.''). 
% We report the proportion of questions for which the model responds ``unanswerable'' when no context is provided.
% ~\cite{neeman2022disentqa} 

% \paragraph{Context sensitivity} 

% \paragraph{Task setup} 

\paragraph{Science QA is more context-sensitive} 
% Since models are more likely to abstain from answering in few-shot settings, 
We assess dataset context sensitivity in the zero-shot setting, when no abstention examples are provided. 
% \lucy{i don't understand why it's reasonable to say that we assess models in the zero-shot setting because they are worse} 
% {\color{red}I don't know if it makes sense. demonstrations in few-shot setting has taught model to refer to context since demonstrations has context or there are examples  abstain from answering, therefore we could not see model's spontaneous behavior whether it will abstain or rely on its own memory .} 
In Table~\ref{tab:noAns_f1_no_context}, we see that a higher proportion of science QA questions (\qasper and \pubmedqa) are answered ``Unanswerable,'' which means these datasets tend to be more context-sensitive than \squad. Because science QA includes more domain-specific terms and concepts that appear infrequently in pretraining data, the models may tend to recognize that without context, they cannot provide an answer. 


% This situation is distinct from puzzles and pure reasoning tasks, which are designed intentionally to be context-independent.  That is, it is conceivable that a scientific question \textit{could} be answerable from parametric knowledge, but empirically it tends \textit{not} to be answerable. 

\paragraph{LLMs vary on answerability} Table~\ref{tab:noAns_f1_no_context} shows that ChatGPT and GPT-3 behave differently for unanswerable questions.  Chatgpt is better at answering unanswerable questions on three datasets. In particular, with no context, ChatGPT achieves 1.0 on the \qasper dataset, which means that it is able to abstain from making uncertain predictions for all questions. GPT-3, in comparison, is much less likely to answer ``unanswerable'' on both \qasper and \pubmedqa regardless of context.

% \noindent\textbf{Science Q&A is more context-sensitive} As shown in figure~\ref{fig:changing_context}, context (even gold evidence) causes performance on unanswerable questions to drop.  That is, providing any context at all, correct or incorrect, tends to increase confidence in answering the question.    Especially in the scientific domain, adding context to the questions can produce a false confidence effect that can cause large language models to incorrectly provide a response rather than correctly abstain.  If the context provided is ambiguous (same paper, random paragraph) rather than irrelevant (random paper, random paragraph), this false confidence effect is more pronounced, as shown in Table~\ref{tab:context_type_qasper}. We posit that ambiguous context is more likely in practice: users will provide information that they believe to be relevant, but may not actually help answer the question.  The model may spur false beliefs in this context.



% \noindent\textbf{LLMs rely more on the context of science Q\&A} As shown in Figure~\ref{fig:changing_context}, 



 % \noindent\textbf{Squad2 is context-insensitive} The performance of gpt-3.5 on Squad2 on unanswerable questions is nearly the same with or without the gold context, as shown in Figure 3. It is probably that squad2 has been contained in the training data of chatgpt and text-davince-002.

















\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
Context type &  none & ext. & abs. & bool.  & all\\ 
\midrule
\multicolumn{6}{c}{\gpt} \\
\midrule
Gold &0.85 &\textbf{0.65}  & \textbf{0.37}& \underline{0.77}  & \textbf{0.63} \\
% \midrule
Ambiguous & \underline{0.88}& \underline{0.56} &0.23  &\textbf{0.79} &0.54 \\
Irrelevant & \textbf{0.96}  & 0.55 & \underline{0.24} & 0.70 &\underline{0.56} \\
Wikipedia  & 0.85 & 0.52 & 0.22 &\textbf{0.79} &0.53 \\
Generated & 0.8 & 0.39 & 0.20 & 0.52 & 0.41 \\
\midrule
\multicolumn{6}{c}{ChatGPT} \\
\midrule
Gold & \underline{0.97}& \textbf{0.56} & \textbf{0.29}&  \textbf{0.69}  & \textbf{0.57}\\
% \midrule
Ambiguous &  \underline{0.97} & 0.50 &0.25  &0.55 &0.52\\
Irrelevant &  \textbf{1.0}  &\underline{0.55}  &  \underline{0.27} & \underline{0.61}  & \underline{0.55}\\
Wikipedia & 0.91  &  0.44 &  0.20& 0.46& 0.47 \\
Generated & 0.85 & 0.40 & 0.12&0.36 & 0.41\\

\bottomrule
\end{tabular}
  \caption{F1 Performance comparison on \qasper dataset when four types of noisy context are added in addition to gold context under the few-shot setting. Bold numbers refer to the best performance in the column. Underlined numbers mean the second-best performance in the column.}
\label{tab:distraction_qasper}
\end{table}






\section{Context Expansion}

\input{tables/context_expansion}

We investigate model distractibility using the \qasper and \pubmedqa datasets. For \qasper, we provide ambiguous context, irrelevant context, retrieved paragraphs from Wikipedia, and paragraphs generated by LLMs as extra context to examine model distractibility. For \pubmedqa, we provide random context, retrieved paragraphs from Wikipedia, and paragraphs generated by LLMs as extra context. Details about how to obtain these context are introduced in Section~\ref{sec:Context_design}.
We evaluate distractibility by measuring the F1 performance change after adding various context. 
For a solution to reduce distraction, we introduce noisy context during ICL to mitigate distractibility. 

\paragraph{Noisy context increases distractibility, in some cases} As shown in Table~\ref{tab:distraction_qasper}, we find that any context provided in addition to gold context generally degrades model performance. However, there are some differences among the types of context, e.g., irrelevant context induces low distractibility for GPT-3 (from 0.65 to 0.55), while generated context causes high distractibility (from 0.65 to 0.39). 
% \lucy{i changed these numbers to match the table, please verify}. 
Although overall performance drops, adding irrelevant context actually increases performance on unanswerable questions. Although retrieval of external knowledge has demonstrated success on other NLP tasks, in our setting, it did not improve performance. We find similar results on \pubmedqa shown in APP.~\ref{app:distractibility}. We also observed that adding more pieces of ambiguous context (Figure~\ref{fig:append_in_paper}) first caused drops in performance before improving performance. Since ambiguous context comes from the same paper, it is not unlikely that some of these passages may provide answers to the question. 

% \noindent\textbf{Distraction effect is highly relevant to answer type} As shown in Figure~\ref{fig:append_in_paper}, abstractive answer is most susceptible to various context. Adding more irrelevant context to questions with abstractive answer can decrease the performance while adding more ambiguous context could improve the performance.

\paragraph{In-context learning with noisy context improves robustness} Adding noisy context in ICL examples consistently and effectively reduces the distractibility of LLMs on \qasper and \pubmedqa. As shown in Figure~\ref{fig:ctx_perturb_gpt}, adding ambiguous or irrelevant context during ICL increases model robustness to most types of noisy context at test time. Similar results on \pubmedqa is included in APP.~\ref{app:distractibility}

% when adding LLM-generated context from 0.41 to 0.50 \lucy{i do not see this in the figure. looks like performance drops for most settings??}.
% {\color{red}In chatgpt, irrelevant context as perturbation works while ambiguous context doesn't work.  In \gpt, both perturbation works.} 

\begin{figure}[t!]
\centering
\includegraphics[width=0.44\textwidth,trim={1cm 0.5cm 1cm 1.3cm},clip]{figure/append_in_paper.pdf}
\caption{F1 change when adding multiple paragraphs of ambiguous context on top of gold context on \qasper using GPT-3.}\label{fig:append_in_paper}
\end{figure}

\begin{figure}[t!]  
\centering
\includegraphics[width=0.44\textwidth,trim={1cm 0.5cm 1cm 1cm},clip]{figure/ctx_perturb_gpt.pdf}
\caption{F1 Performance comparison on \qasper dataset about adding four type of context (ambiguous, irrelevant, wikipedia, generated) on the top of gold context under three ways of demonstrations in ICL (gold context, gold context with irrelevant context, gold context with ambiguous context) using GPT-3. 
}\label{fig:ctx_perturb_gpt}
\end{figure}



==> old/intro.tex <==
\section{Introduction}


\begin{figure}[t]
\centering
\minipage{\linewidth}
\includegraphics[width=\linewidth]{figure/framework.pdf}
\caption{Our proposed framework to probe the context sensitivity of LLMs for science QA. 
% \lucy{Good! font needs to be a bit bigger and would be good to indicate that the answer to the question is in document A}
}\label{fig:prompts_format}
\endminipage
\end{figure}

% Large language models(LLMs) \citep{brown2020language, wei2021finetuned,chowdhery2022palm,chung2022scaling} have produced striking results on natural language processing tasks, particularly in knowledge-intensive tasks ~\cite{yu_generate_2022}.  Efforts to understand these results have shown that parametric knowledge encoded from the training set is frequently responsible, even when the results appear to demonstrate reasoning~\cite{wei2022chain,zhou2022least}.  
% Tasks ranging from fully parametric (e.g., general knowledge facts easily answerable with the public internet) to pure reasoning (e.g., logic problems or arithmetic) have varying degrees of context-sensitivity: the degree to which user-provided information is required to answer the question.  Parametric knowledge is unreliable in context-sensitive situations: LLMs may encode misconceptions or obsolete facts~\cite{kasai2022realtime} and yield a wrong answer when the retrieved documents are outdated or unrelated. In these cases we expect LLMs to \emph{correct} their predictions when provided with relevant context. These relevant context could come from datasets, general sources like Wikipedia through various retrieval models~\cite{khattab2022demonstrate, zhong2022training,gao-callan-2022-unsupervised,guu2020retrieval,shi2023replug} or generated knowledge from the memory of the model~\cite{yu_generate_2022}

% \lucy{make sure all dataset names and spellings are consistent. i created a few commands for this \squad \pubmedqa \qasper \gpt which should help} 

% Science QA tasks ask models to answer questions from an informational context. LLMs have been successfully applied to a range of science QA tasks \todocite

% Solving Impressed by the remarkable ability of LLMs' in-context-learning approach, many qa tasks take LLM as reader~\cite{wei2022chain,zhou2022least} to understand given context. But LLMs

% Even though parametric knowledge and contextual knowledge are widely used, only a few studies addressed the relation between them in the context of LLMs. 

Large language models (LLMs) have enabled rapid progress on knowledge-intensive tasks such as scientific question answering (QA). LLMs demonstrate remarkable few-shot capabilities \cite{brown2020language} to generate accurate answers based on provided informational contexts. However, the influence of incorrect context on LLM performance in scientific QA tasks remains a relatively unexplored area of research. Recent studies have shown that LLMs can be distracted by irrelevant context~\citep{shi2023large}. Prior work has identified challenges such as entity-based knowledge conflicts~\cite{longpre-etal-2021-entity} and model inability to make predictions with abstention~\cite{neeman2022disentqa, zhou2023context}. 
% \citet{zhou2023context} propose prompting methods to improve model faithfulness to context. 

% However, in the scenarios with long context contained with high expertise, large language model behave differently. 

In this paper, we study LLM context sensitivity in science QA tasks. We investigate model ability to make predictions with \emph{abstention} as well as model \emph{distractibility} when provided with irrelevant or incorrect context. We define prediction with abstention as a model correctly abstaining from answering a question when no or incorrect context is provided in a document-based QA setting. Distractibility is whether a model is impacted by irrelevant context. We introduce a framework for prompting LLMs with different types of context to explore these two behaviors. We examine the effectiveness of our framework by testing two GPT-family LLMs with different contexts in one general domain and two scientific domain QA datasets: \squad, \pubmedqa, and \qasper. 

% We prompt two GPT-family LLMs with different contexts.  Prediction with abstention refers to that how large language models handle with unanswerable questions from no context to context with different quality.  We develop a new framework by prompting LLMs using various type of context to better evaluate model's prediction with abstention and distractibility. 

We summarize our contributions below:
%more bullit about findings
\begin{itemize}[itemsep=0.2pt, topsep=3pt, leftmargin=10pt]
    \item We introduce a framework to study LLM sensitivity to different types of input context for science QA. Specifically, we probe (i) LLM ability to predict with abstention and (ii)LLM ability to deal with context expansion.
    % We hope this work will give an insight to the community about dealing with scientific question answering tasks. We incorporate context-insensitive tasks (factoid QA) and context-sensitive tasks (document-based science QA). 
    \item Using this framework, we investigate the context-sensitivity of ChatGPT and GPT-3 on three QA datasets, ranging from context-insensitive tasks like factoid QA to context-sensitive tasks like document-based science QA. We find that both models are sensitive to different types of context. While ChatGPT is better at abstaining for unanswerable questions, GPT-3 achieves better performance across other question types. GPT-3 is more distracted by irrelevant context than ChatGPT, though providing irrelevant contexts during in-context learning improves performance robustness for both models.
    
    % \item For context perspective, science qa is more context-sensitive than general qa. And all context variants regardless of relevance cause different level of distractibility for LLMs even given gold context.

    % \item From model's perspective, chatgpt is better at answer unanswerable questions compared with \gpt while \gpt achieves higher performance on other question types. Chatgpt experiences less distractibility than \gpt  given the same context.  We could consider mixture of experts methods to combine various LLMs' advantages.
    
    
    % For distractibility, we analyze four type of context (ambiguous, irrelevant, from wikipedia, LLM-generated) cause different level of distractibility for LLMs even given gold context.  Also, distractibility is highly relevant to answer types (extractive, abstractive, boolean and unanswerable). Furthermore, we present context perturbation strategies to reduce distractibility.
\end{itemize}


 









==> old/limitation.tex <==
\section*{Limitation}
We only explore two prompting strategies. Future work should explore more prompting methods such as least-to-most prompting and program prompting. In the few-shot setting, we adopt KNN approach to select similar examples to use in ICL and only use up to three examples. More examples and better example selection methods may improve performance.

We only perform experiments with two LLMs (both GPT-family), and consequently, our results may not generalize to other LLMs. We encourage the use of our framework to investigate context sensitivity in other language models.


% In this work, we only show results of two LLMs (chatgpt and \gpt) and three datasets (squad2, pubmedqa and qasper). We will include more LLMs and datastes in the future. \lucy{this will get us desk rejected} 

==> old/method.tex <==





% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
%   datasets & \multicolumn{3}{c}{ChatGPT (zero/few shot)} & \multicolumn{3}{c}{text-davinci-002 (zero/few shot)} & \multicolumn{3}{c}{Flan-T5-xl (zero/few shot)}   \\ 
% \midrule 
% % & \multicolumn{9}{c}{zero-shot/few-shot} \\
% % \midrule 
%    & noANS & HasANS & ALL & noANS & HasANS & ALL& noANS & HasANS & ALL \\
%    \midrule
% % wikiQA &    0.16  & 0.07& 0.07 &0.46/  & 0.17/&0.17/  &  \\
% squad2  &   0.48/  & 0.25/&0.48/ & 0.53 &0.42 &  0.53\\ 
% pubmedQA & 0.59/0.78 &0.44/0.78 & 0.46/0.78 & 0.04/0.15 &0.01/0.05 & 0.03/0.06 & \textbf{0.0} &\textbf{0.0} & \textbf{0.0}\\
% qasper  & \textbf{1.0/0.95} & \textbf{1.0/0.88}  & \textbf{1.0/0.98} & 0.94/0.92  &0.81/0.67  & 0.95 /0.88 & 0.91/0.86  &0.56/0.47 &0.88/0.81 \\
% \bottomrule
% \end{tabular}
%   \caption{ Unanswerability evaluation on four various datasets with no context.}
% \label{tab:noAns_f1_no_context}
% \end{table*}


% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
%  datasets & \multicolumn{3}{c}{ChatGPT (zero/few shot)} & \multicolumn{3}{c}{text-davinci-002 (zero/few shot)} &\multicolumn{3}{c}{Flan-T5-xl (zero/few shot)}   \\ 
% \midrule 
% % & \multicolumn{9}{c}{zero-shot/few-shot} \\
% % \hline 
%    & noANS & HasANS & ALL & noANS & HasANS & ALL & noANS & HasANS & ALL \\
%    \midrule
% % wikiQA &   0.47/   & 0.17/ &0.17/ & 0.40/&   0.17/&  0.17/&  \\
% squad2  &   0.42/  & 0.03/ &0.42/ & 0.27/ &0.03/ &0.27/  \\
% pubmedQA & 0.33/0.56 &0.25/0.52 &0.26/0.52 & 0.18/0.33 & 0.13/0.21& 0.14/0.22 & \textbf{0.0} &\textbf{0.0} & \textbf{0.0}\\
%  qasper  &  1.0/0.94 &0.21/0.29  & 0.10/0.14 & 0.97/0.89  &0.23/0.08 &  0.13/0.04 & 0.88/0.85  &0.12/0.11 &0.22/0.28 \\
% \bottomrule
% \end{tabular}
%   \caption{ Unanswerability evaluation on four various datasets with gold context. }
% \label{tab:noAns_f1_with_context}
% \end{table*}


\begin{table}[t!]
\centering
\small
\begin{tabular}{p{13mm}p{10mm}p{9mm}p{15mm}p{8mm}}
\toprule
 Dataset & Context length & Unans. ratio & Answer types & Testset Size \\ 
\midrule 
\squad  &   128  & 0.5 & Ext & 11873\\
\pubmedqa   &  204 & 0.1 & Bool &  500\\
\qasper  & 226 & 0.1 & Ext/Abs/Bool & 1451\\
BioASQ  & 270 & 0.0 & Bool & 140\\
\bottomrule
\end{tabular}
  \caption{Dataset statistics.}
\label{tab:datasets}
\end{table}

\input{tables/answerc_change}
\input{tables/model_unanserability}
\input{tables/model_answerability}

\section{Framework}

% The input of these tasks is formulated as (context, question) for free-form generation tasks. The desired output could be a free-form answer, extractive span in the context, boolean(yes/no) or unanswerable.


\subsection{Prompting strategies} 
In this work, we test two common prompting strategies: zero-shot and few-shot instruction prompting. 
% Our framework also supports other prompting methods. 

\begin{itemize}[itemsep=0pt, topsep=2pt, leftmargin=0pt]
    \item[] \textbf{Zero-shot}: Given an input pair $(c, q)$ where $c$ is context and $q$ is question, we prepend the instruction (App.~\ref{app:prompt_templates}) with an explicit directive for handling unanswerable questions.
    \item[] \textbf{Few-shot}: In-context learning (ICL) has been successfully adapted for many NLP tasks, and mitigates the need for additional model training or finetuning \citep{brown2020language}. Following \citet{liu-etal-2022-makes}, we adopt KNN to select similar questions in the training dataset to provide as ICL examples; we use ColBERTv2~\cite{santhanam-etal-2022-colbertv2} as our retriever. Inspired by chain-of-thought prompting~\cite{wei2022chain}, we ask models to generate explanations first before answering the question (full prompt templates in App.~\ref{app:prompt_templates}).
\end{itemize}

% \paragraph{Zero-shot setting} Given an input pair $(c, q)$ where $c$ is context and $q$ is question, we prepend the instruction (App.~\ref{app:prompt_templates}) with an explicit directive for handling unanswerable questions.
% % (we begin with the following zero-shot prompting template and use explicit instructions to handle with unanswerable questions shown in Figure~\ref{fig:0shot_demo}.

% \paragraph{Few-shot setting} In-context learning (ICL) has been successfully adapted for many NLP tasks, and mitigates the need for additional model training or finetuning \citep{brown2020language}. Following \citet{liu-etal-2022-makes}, we adopt KNN to select similar questions in the training dataset to provide as ICL examples; we use ColBERTv2~\cite{santhanam-etal-2022-colbertv2} as our retriever.
% % , a state-of-the-art retriever based on late interaction~\cite{khattab2020colbert}, 
% % to retrieve the top three similar questions based on embedding cosine similarity. 
% % We choose ColBERTv2 for its highly effective zero-shot search quality and efficient search~\cite{santhanam-etal-2022-colbertv2}. 
% Inspired by chain-of-thought prompting~\cite{wei2022chain}, we ask models to generate explanations first before answering the question (full prompt templates in App.~\ref{app:prompt_templates}).



\subsection{Context Design}\label{sec:Context_design}
% In this work, we focus on the context sensitivity of large language models. Hence apart from provided context, we create some variants of context from parametric knowledge or non-parametric knowledge to access LLMs. 
We use the following types of context to probe model sensitivity to context.

\begin{itemize}[itemsep=0pt, topsep=2pt, leftmargin=0pt]
    \item[] \textbf{Given}: Given context from dataset.
    \item[] \textbf{Random}: We randomly sample other question contexts to provide in the test setting.
    % \item[] \textbf{Ambiguous}: We randomly sample paragraphs from the same paper of the test example, excluding any gold paragraphs. This setting is only used for \qasper.
    % % excluding the gold paragraphs as ambiguous context.
    % \item[] \textbf{Irrelevant}: We randomly sample paragraphs from a different paper as irrelevant context. This setting is only used for \qasper and is equivalent to the Random setting for other datasets.   
    \item[] \textbf{Wikipedia}: Retrieval has been shown to assist LLMs in knowledge-intensive QA~\cite{khattab2022demonstrate, zhong2022training,gao-callan-2022-unsupervised,guu2020retrieval,shi2023replug}. We investigate how retrieved Wikipedia paragraphs affect model performance. We use Contriever~\cite{izacard2021contriever} as our retrieval model.
    \item[] \textbf{Generated}: Genread~\cite{yu_generate_2022} shows that knowledge generated by LLMs is competitive with retrieved knowledge in improving knowledge-intensive QA performance in the general domain. We apply Genread~\cite{yu_generate_2022} to generate background paragraphs. The prompt template is ``please provide a background document to the question.''
\end{itemize}




\subsection{Models}
\label{sec:models}
Our framework supports various LLMs. In this work, we conduct experiments using ChatGPT and GPT-3 (\gpt). 
% We prompt these models in zero-shot and few-shot settings. 
For both models, we set the temperature to 0 and top-p sampling to 1 to reduce the variability of model output. 

\subsection{Datasets}
\label{sec:datasets}
% We evaluate LLMs’ ability to selectively abstain from making uncertain predictions on existing datasets using various context. 
We conduct experiments on three QA datasets: \squad~\cite{rajpurkar-etal-2018-know}, \pubmedqa~\cite{jin-etal-2019-pubmedqa}, and \qasper~\cite{dasigi2021dataset}. Dataset details are provided in Table~\ref{tab:datasets} and App.~\ref{app:dataset_details}. \squad is a general-domain factoid QA dataset, while \pubmedqa and \qasper are science QA datasets with contexts derived from scientific papers. \qasper is document-based, with all questions only answerable from an associated document. These datasets generally have long contexts (>100 words) and all contain ``unanswerable'' questions.  
 




==> old/related_work.tex <==

\section{Related Work}

\paragraph{Prompting LLMs in science QA} The few-shot capability of LLMs has emerged as a powerful approach for addressing knowledge-intensive tasks like question answering~\citep{brown2020language, wei2021finetuned, chowdhery2022palm}. Recent prompting strategies such as chain-of-thought (CoT)~\citep{wei2022chain}, least-to-most (LTM)~\citep{zhou2022least}, and others~\citep{kojima2022large,wang2022self} significantly improve LLMs' zero or few-shot abilities on diverse QA benchmarks in the general~\cite{rajpurkar-etal-2018-know, yang-etal-2015-wikiqa} and scientific~\cite{jin-etal-2019-pubmedqa,dasigi2021dataset} domains. \citet{pereira2023visconde} adopt 
retrieve-than-read on the \qasper dataset~\cite{dasigi2021dataset} and show that current retrievers are the main bottleneck and that readers (LLMs) are already performing at the human level as long as relevant passages are provided. Inspired by this finding, we are interested in how irrelevant or incorrect contexts can impact LLM performance on context-intensive QA tasks. 
% On the other hand, \cite{lu2022learn} bring multi-modality context into science QA. However, we only focus on text in this work. We will leave multi-modality context as future work.


% \noindent\textbf{Contextual and parametric knowledge} Large language models~\cite{brown2020language, wei2021finetuned, chowdhery2022palm} has demonstrated remarkable ability in memorizing factual information in closed book QA tasks using their parameters. These parametric memory is acquired during pretraining on the large-scale corpus. However, solely relying on parametric knowledge to do make prediction has several limitations: the memorized factual information is easily outdated and  an unseen new fact may lead to an incorrect or poor prediction~\cite{lazaridou2021mind, kasai2022realtime}. To overcome these limitations, one promising direction is to leverage contextual knowledge using prompting strategies to enhance LMs’ abilities on knowledge-intensive tasks. Contextual knowledge could come from external resources~\cite{khattab2022demonstrate, zhong2022training,gao-callan-2022-unsupervised,guu2020retrieval,shi2023replug} or model memorization~\cite{yu2022generate}. Even though these two very different knowledge sources are widely used, only a few studies addressed the relation between them in the context of LLMs. \cite{longpre-etal-2021-entity} shows that LLMs easily ignore context and refers to model's own parametric knowledge. To tackle this challenge, \cite{li2022large} finetune LLMs on counterfactual contexts and effectively improve the LLMs’ utilization of contexts instead of relying solely on their parametric knowledge. \cite{neeman2022disentqa} also use counterfactual data augmentation and further disentangle contextual knowledge and parametric knowledge in a way that predicting two answers based on these two kind of knowledge respectively for a given question. It could to some extent alleviate knowledge conflict problem. More recent study \cite{zhou2023context} adopt opinion-based prompts and counterfactual demonstrations to solve knowledge conflict. Apart from letting model pay attention to relevant context, some studies find that irrelevant context causes trouble for LLMs. \cite{zhou2023context} believe that we should do prediction with abstention when provided context is irrelevant. \cite{shi2023large} find the model performance is dramatically decreases when irrelevant information is included.

% Although previous work has studies some aspects of contextual and parametric knowledge, they are lack of in-depth analysis of different type of context(e.g., no context, irrelevant, ambiguous context, gold context). Furthermore, they mainly focus on context in general domain and neglect context in scientific domain. In this work, we propose a framework to probe large language models' ability to understand various type of context from general domain to scientific domain. 
\paragraph{Unanswerability in LLMs} Several works have recently shown that LLMs become easier to steer with natural language prompts either as they become larger~\cite{mishra-etal-2022-reframing} or as they are exposed to larger instruction tuning data~\cite{mishra-etal-2022-cross,chung2022scaling}, and as a consequence, it might improve the unanswerability capabilities of the model. Specifically, in this work, we utilize prompt manipulation in order to systematically reveal to the model the option of avoiding answering hard questions. Automatic prompt tuning can be also used for improving unanswerability capabilities, without the need for manual handcrafting prompts. \citet{liao2022ptau} introduced a prompt tuning-based strategy to mitigate unanswerable questions, by mapping questions into their proper, specific templates.

Other works tried to manipulate the model predictions towards better unanswerability via using data augmentation \cite{zhu-etal-2019-learning}, and \citet{asai-choi-2021-challenges} provided an in-depth analysis of the ability to detect unanswerability in LMs, where the case study is the data which is fed to the model. 





\paragraph{Perturbing contexts}  Prior work studying input perturbations for NLP tasks include approaches such as model-agnostic input transformations~\cite{liang2022holistic, ravichander2022condaqa} and adversarial example generation~\cite{jia2017adversarial, wang2021adversarial}. \citet{liang2022holistic} use input transformations including semantics-preserving and semantics-altering perturbations, in their robustness evaluation of LLMs. Other work has shown that pretrained language models are negatively impacted by irrelevant context~\cite{chowdhery2022palm, liang2022holistic}.
In particular, \citet{liang2022holistic} evaluated T5~\cite{raffel2020exploring} and PaLM~\cite{chowdhery2022palm} using few-shot prompting, and demonstrated that finetuning these models with counterfactual and irrelevant contexts improves model robustness to noisy context. In our framework, we show that without training or finetuning, adding noisy context in in-context learning examples also improves model robustness.
% mitigates the distractibility of the underlying language model and significantly improves the model performance on our scientific context benchmark.


==> old/tables.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{p{13mm}p{10mm}p{9mm}p{15mm}p{8mm}}
\toprule
 Dataset & Context length & Unans. ratio & Answer types & Testset Size \\ 
\midrule 
WIKIQA &    212 & 0.6 & Ext &  6165\\
\squad  &   128  & 0.5 & Ext & 11873\\
\pubmedqa   &  204 & 0.1 & Bool &  500\\
\qasper  & 226 & 0.1 & Ext/Abs/Bool & 1451\\
BioASQ  & 270 & 0.0 & Bool & 140\\
\bottomrule
\end{tabular}
  \caption{Dataset statistics.}
\label{tab:datasets}
\end{table}



\begin{table}[t!]
\scriptsize
\centering
\begin{tabular}{lcccc}
\toprule
   & \multicolumn{2}{c}{ChatGPT} & \multicolumn{2}{c}{\gpt}   \\ 
\midrule 
% & \multicolumn{9}{c}{zero-shot/few-shot} \\
% \midrule 
   Dataset & NoANS & HasANS  & NoANS & HasANS  \\
   \midrule
% wikiQA &    0.16  & 0.07& 0.07 &0.46/  & 0.17/&0.17/  &  \\
\squad  &   \textbf{0.63}/1.0  & \textbf{0.53}/0.99 & \textbf{0.59}/0.89 & \textbf{0.40}/0.87 \\ 
\pubmedqa & \textbf{0.89}/0.41 & \textbf{0.84}/0.69  & \textbf{0.59}/0.63 &\textbf{0.61}/0.77  \\
\qasper  & \textbf{\underline{0.98}}/1.0 & \textbf{\underline{0.93}}/1.0   & \textbf{\underline{0.89}}/0.97  &\textbf{\underline{0.75}}/0.83   \\
\bottomrule
\end{tabular}
  \caption{Answerability with no context (zero/few-shot). Higher number means more questions are answered  ``unanswerable''. Bold numbers are zero-shot performance. Underlined numbers refer to the highest answerability in the zero-shot column.}
\label{tab:noAns_f1_no_context}
\end{table}



% \begin{table*}[t]
% \small
% \centering
% \begin{tabular}{c|ccc|ccc}
% \toprule
%   datasets & \multicolumn{3}{c}{ChatGPT (zero/few shot)} & \multicolumn{3}{c}{text-davinci-002 (zero/few shot)}   \\ 
% \midrule 
% % & \multicolumn{9}{c}{zero-shot/few-shot} \\
% % \midrule 
%    & noANS & HasANS & ALL & noANS & HasANS & ALL \\
%    \midrule
% % wikiQA &    0.16  & 0.07& 0.07 &0.46/  & 0.17/&0.17/  &  \\
% squad2  &   0.48/  & 0.25/&0.48/ & 0.53 &0.42 &  0.53\\ 
% pubmedQA & 0.59/0.78 &0.44/0.78 & 0.46/0.78 & 0.04/0.15 &0.01/0.05 & 0.03/0.06 \\
% qasper  & \textbf{0.98/1.0} & \textbf{0.93/1.0}  & \textbf{0.94/1.0} & 0.94/0.92  &0.81/0.67  & 0.95 /0.88 \\
% \bottomrule
% \end{tabular}
%   \caption{ Answerability evaluation on three various datasets with no context.}
% \label{tab:noAns_f1_no_context}
% \end{table*}



% \begin{figure}[t!]
% \centering
% \minipage{0.5\textwidth}
% \includegraphics[width=\linewidth]{figure/0to1.pdf}
% \caption{Performance change on unanswerable questions from no context to gold context using chatgpt under few-shot setting.}\label{fig:changing_context}
% \endminipage
% \end{figure}


% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{ccccc}
% \toprule
% context type &  none & ext. & abs. & bool. \\
% \midrule
% \multicolumn{5}{c}{chatgpt} \\
% \midrule
% No context &  0.98 & 0.98 &0.94  &0.75\\
% Irrelevant &  1.0  & 0.90 &0.91&0.70 \\
% Ambiguous   &  1.0 & 0.83 & 0.91 &0.67   \\
% Gold context & 0.94 & 0.14 & 0.43 &0.29\\
% \midrule
% \multicolumn{5}{c}{text-davinci-002} \\
% \midrule
% No context &  0.92  & 0.88 & 0.73 &0.42\\
% Irrelevant &   0.73 & 0.63 & 0.69 &0.42  \\
% Ambiguous   &   0.55 & 0.49 & 0.44 &0.38   \\
% Gold context & 0.89* & 0.04 & 0.16 &0.07\\
% \bottomrule
% \end{tabular}
%   \caption{Answerability evaluation on qasper dataset. Given irrelevant and bad context, the percentage of questions that are answered ``unanswerable'' for each question type in few-shot setting. *No context is provided as gold.}
% \label{tab:context_type_qasper}
% \end{table}


% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{ccccc}
% \toprule
%  &  No  & Irr. & Amb. & Gold   \\
% \midrule
% ChatGPT &  0.98&  1.0  &  1.0& 0.97 \\
% \gpt &  0.97  &   0.91 &   0.86 & 0.89* \\
% \bottomrule
% \end{tabular}
%   \caption{Answerability for unanswerable questions in the \qasper dataset, when different contexts are provided to the model. 
%   % Given irrelevant and bad context, the percentage of questions that are answered ``unanswerable'' for each question type in few-shot setting. 
%   *No context is provided as gold. \lucy{what is difference between No and Gold?}
% unanswerable questions' gold context is just empty so there is no difference. \lucy{then why is the score different?} because in qasper evaluation, some questions could be have many annotations. their types are based on their maximum-F1 answers}
% \label{tab:context_type_qasper}
% \end{table}




% \section{Experiment}

% This section presents our experimental setup (\S\ref{sec:experimental_setup}) for the evaluation of the proposed framework concerning two aspects: prediction with abstention(§4.2) and distractibility (§4.3).

% \subsection{Experimental Setup}
% \label{sec:experimental_setup}
% Our experiments are conducted using chatGPT and text-davinci-002. We conduct experiments in two different settings: zero-shot and few-shots settings. We set the temperature as 0 and top p sampling as 1 to decrease the randomness of model output. \lucy{move models to end of section 3 and create two sections for prediction with abstention and distractibility; the current organization is too messy (with the nested results sections)}

\section{Prediction with abstention}
\label{sec:prediction_w_abstention}

We introduce the concept of context-sensitivity to estimate the extent of context-dependence of our three QA datasets given a particular model. We measure context-sensitivity by removing all context from all questions and asking models to provide answers. The proportion of questions for which the model abstains (i.e., predicts ``unanswerable'') is interpreted as the context-sensitivity of the dataset from the perspective of the given model. The intuition is that if a model tends to use parametric knowledge to answer a question without context, correctly or incorrectly, then the model does not consider the question to be context-sensitive. A dataset that has many such questions is itself considered to be less context-sensitive. 
% \lucy{what is the relationship between context-sensitivity, answerability, and prediction with abstention? not sure what i'm supposed to get out of this section with some many terms and definitions} Answerability is defined as the as accuracy for predicting the special token “unanswerable” given no context or random context. I would say these three are equal. We could just use one to unify the terms. high answerability = context-sensitivity  = prediction with abstention \lucy{+1 please combine to reduce confusion}

If a dataset is context-sensitive, then answerable questions within the dataset should become unanswerable if the context is removed. We test this by reporting the proportion of questions in each dataset for which the model responds ``unanswerable'' when no context is provided. We report results in Table~\ref{tab:noAns_f1_no_context}; HasAns are questions for which a context-dependent answer is provided in the dataset, and NoAns are questions the dataset labels as unanswerable.
% , 
% we report model context-sensitivity
% \lucy{what is answerability score? Answerability is defined as the as accuracy for predicting the special token “unanswerable” given no context or random context} 
% on the questions for which a (context-dependent) answer is provided in the dataset (HasAns), and on questions for which no answer is provided in the dataset (NoAns) (i.e., the ground truth response is ``unanswerable.''). 
% We report the proportion of questions for which the model responds ``unanswerable'' when no context is provided.
% ~\cite{neeman2022disentqa} 

% \paragraph{Context sensitivity} 

% \paragraph{Task setup} 

\paragraph{Science QA is more context-sensitive} 
% Since models are more likely to abstain from answering in few-shot settings, 
We assess dataset context sensitivity in the zero-shot setting, when no abstention examples are provided. 
% \lucy{i don't understand why it's reasonable to say that we assess models in the zero-shot setting because they are worse} 
% {\color{red}I don't know if it makes sense. demonstrations in few-shot setting has taught model to refer to context since demonstrations has context or there are examples  abstain from answering, therefore we could not see model's spontaneous behavior whether it will abstain or rely on its own memory .} 
In Table~\ref{tab:noAns_f1_no_context}, we see that a higher proportion of science QA questions (\qasper and \pubmedqa) are answered ``Unanswerable,'' which means these datasets tend to be more context-sensitive than \squad. Because science QA includes more domain-specific terms and concepts that appear infrequently in pretraining data, the models may tend to recognize that without context, they cannot provide an answer. 


% This situation is distinct from puzzles and pure reasoning tasks, which are designed intentionally to be context-independent.  That is, it is conceivable that a scientific question \textit{could} be answerable from parametric knowledge, but empirically it tends \textit{not} to be answerable. 

\paragraph{LLMs vary on answerability} Table~\ref{tab:noAns_f1_no_context} shows that ChatGPT and GPT-3 behave differently for unanswerable questions.  Chatgpt is better at answering unanswerable questions on three datasets. In particular, with no context, ChatGPT achieves 1.0 on the \qasper dataset, which means that it is able to abstain from making uncertain predictions for all questions. GPT-3, in comparison, is much less likely to answer ``unanswerable'' on both \qasper and \pubmedqa regardless of context.

% \noindent\textbf{Science Q&A is more context-sensitive} As shown in figure~\ref{fig:changing_context}, context (even gold evidence) causes performance on unanswerable questions to drop.  That is, providing any context at all, correct or incorrect, tends to increase confidence in answering the question.    Especially in the scientific domain, adding context to the questions can produce a false confidence effect that can cause large language models to incorrectly provide a response rather than correctly abstain.  If the context provided is ambiguous (same paper, random paragraph) rather than irrelevant (random paper, random paragraph), this false confidence effect is more pronounced, as shown in Table~\ref{tab:context_type_qasper}. We posit that ambiguous context is more likely in practice: users will provide information that they believe to be relevant, but may not actually help answer the question.  The model may spur false beliefs in this context.



% \noindent\textbf{LLMs rely more on the context of science Q\&A} As shown in Figure~\ref{fig:changing_context}, 



 % \noindent\textbf{Squad2 is context-insensitive} The performance of gpt-3.5 on Squad2 on unanswerable questions is nearly the same with or without the gold context, as shown in Figure 3. It is probably that squad2 has been contained in the training data of chatgpt and text-davince-002.

\begin{table}[t]
\centering
\small
\begin{tabular}{lcc}
\toprule
Model &  none & extractive  \\ 
\midrule
\multicolumn{3}{c}{no context} \\
\midrule
Flan-t5-xl &0.90 & 0.88    \\
% \midrule
Llamav2-13b-chat & 0.56& 0.17\\
vicuna1.5-13b-chat& 0.37  & 0.21  \\
GPT3.5  & 0.968 & 1.0 \\
text-davince-002 &  0.992 & 0.968\\
\midrule
\multicolumn{3}{c}{context} \\
\midrule
Flan-t5-xl &0.88 &0.10 \\
% \midrule
Llamav2-13b-chat &0.76 & 0.17  \\
vicuna1.5-13b-chat &  59.7 &1.80  \\
GPT3.5  & 56.3&27.9  \\
text-davince-002  & 63.9&30.4\\
\bottomrule
\end{tabular}
  \caption{NoAns ratio performance on squad2 dataset under no context and context settings using various LLMs}
\label{tab:distraction_qasper}
\end{table}



\begin{table}[t]
\centering
\small
\begin{tabular}{lccc}
\toprule
Model &  none & yes & no \\ 
\midrule
\multicolumn{4}{c}{no context} \\
\midrule
Flan-t5-xl &0.0 & 0.0  & 0.0 \\
% \midrule
Llamav2-13b-chat & 0.0& 0.0&0.0\\
vicuna1.5-13b-chat& 0.0  & 0.0 & 0.0 \\
GPT3.5  & 88.9& 79.8&90.6 \\
text-davince-002 & 59.3&68.8&49.4  \\
\midrule
\multicolumn{4}{c}{context} \\
\midrule
Flan-t5-xl &0.0 &0.0& 0.0 \\
% \midrule
Llamav2-13b-chat &0.0 & 0.0 &0.0 \\
vicuna1.5-13b-chat& 0.037  & 0.036 & 0.059  \\
GPT3.5  & 55.6& 33.3&61.2 \\
text-davince-002  & 25.9&21.0&17.6 \\
\bottomrule
\end{tabular}
  \caption{NoAns ratio performance on pubmedQA dataset under no context and context settings using various LLMs}
\label{tab:distraction_qasper}
\end{table}



\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
Model &  none & ext. & abs. & bool.  \\ 
\midrule
\multicolumn{6}{c}{no context} \\
\midrule
Flan-t5-xl &0.90 & 0.88  & 0.79& 0.0  &  \\
% \midrule
Llamav2-13b-chat & 0.77& 0.63&0.41& 0.10&\\
vicuna1.5-13b-chat& 0.37  & 0.21 & 0.22 & 0.19 & \\
GPT3.5  &1.0&0.971&0.956&0.889 \\
text-davince-002 & 0.895 & 0.863&0.933&0.2 \\
\midrule
\multicolumn{6}{c}{context} \\
\midrule
Flan-t5-xl &0.88 &0.10& 0.22 & 0.03  & \\
% \midrule
Llamav2-13b-chat &0.76 & 0.17 &0.4 &0.06 & \\
vicuna1.5-13b-chat &  0.32 &0.04  &  0.16 & 0.03   & \\
GPT3.5  &1.0&0.105&0.314&0.214  \\
text-davince-002  & 0.967&0.125&0.354&0.214\\
\bottomrule
\end{tabular}
  \caption{NoAns ratio performance on qasper dataset under no context and context settings using various LLMs}
\label{tab:distraction_qasper}
\end{table}







\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
Context type &  none & ext. & abs. & bool.  & all\\ 
\midrule
\multicolumn{6}{c}{\gpt} \\
\midrule
Gold &0.85 &\textbf{0.65}  & \textbf{0.37}& \underline{0.77}  & \textbf{0.63} \\
% \midrule
Ambiguous & \underline{0.88}& \underline{0.56} &0.23  &\textbf{0.79} &0.54 \\
Irrelevant & \textbf{0.96}  & 0.55 & \underline{0.24} & 0.70 &\underline{0.56} \\
Wikipedia  & 0.85 & 0.52 & 0.22 &\textbf{0.79} &0.53 \\
Generated & 0.8 & 0.39 & 0.20 & 0.52 & 0.41 \\
\midrule
\multicolumn{6}{c}{ChatGPT} \\
\midrule
Gold & \underline{0.97}& \textbf{0.56} & \textbf{0.29}&  \textbf{0.69}  & \textbf{0.57}\\
% \midrule
Ambiguous &  \underline{0.97} & 0.50 &0.25  &0.55 &0.52\\
Irrelevant &  \textbf{1.0}  &\underline{0.55}  &  \underline{0.27} & \underline{0.61}  & \underline{0.55}\\
Wikipedia & 0.91  &  0.44 &  0.20& 0.46& 0.47 \\
Generated & 0.85 & 0.40 & 0.12&0.36 & 0.41\\

\bottomrule
\end{tabular}
  \caption{F1 Performance comparison on \qasper dataset when four types of noisy context are added in addition to gold context under the few-shot setting. Bold numbers refer to the best performance in the column. Underlined numbers mean the second-best performance in the column.}
\label{tab:distraction_qasper}
\end{table}




% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{lccccc}
% \toprule
% Context type &  none & ext. & abs. & bool.  & all\\ 
% \midrule
% \multicolumn{6}{c}{Adding ambiguous context} \\
% \midrule
% gold & 0.93& 0.56 & 0.25&  0.60  & 0.55\\
% Ambiguous & 0.97&0.53&0.19&0.54&0.52\\
% Irrelevant &  0.91&0.46 &0.21 &0.63 & 0.49\\
% From Wikipedia  & 0.94 &0.39&0.16&0.39&0.44    \\
% LLM-generated & 0.85&0.41&0.13&0.5&0.44 \\
% \midrule
% \multicolumn{6}{c}{Adding irrelevant context} \\
% \midrule
% gold & 0.95& 0.57 & 0.22&  0.6  & 0.59\\
% Ambiguous & 0.96&0.53&0.27&0.62&0.54 \\
% Irrelevant &  1.0&0.54 &0.25 &0.54 & 0.54\\
% From Wikipedia  & 0.92 &0.45&0.19&0.39&0.46    \\
% LLM-generated & 0.85&0.41&0.13&0.5&0.44 \\
% \bottomrule
% \end{tabular}
%   \caption{F1 Performance comparison on Qasper dataset between four type of context on the top of gold context when adding ambiguous and irrelevant context as perturbation to the context of demonstrations.  chat-gpt under few-shot setting (will change to figure)}
% \label{tab:context type}
% \end{table}











\section{Context Expansion}

We investigate model distractibility using the \qasper and \pubmedqa datasets. For \qasper, we provide ambiguous context, irrelevant context, retrieved paragraphs from Wikipedia, and paragraphs generated by LLMs as extra context to examine model distractibility. For \pubmedqa, we provide random context, retrieved paragraphs from Wikipedia, and paragraphs generated by LLMs as extra context. Details about how to obtain these context are introduced in Section~\ref{sec:Context_design}.
We evaluate distractibility by measuring the F1 performance change after adding various context. 
For a solution to reduce distraction, we introduce noisy context during ICL to mitigate distractibility. 

\paragraph{Noisy context increases distractibility, in some cases} As shown in Table~\ref{tab:distraction_qasper}, we find that any context provided in addition to gold context generally degrades model performance. However, there are some differences among the types of context, e.g., irrelevant context induces low distractibility for GPT-3 (from 0.65 to 0.55), while generated context causes high distractibility (from 0.65 to 0.39). 
% \lucy{i changed these numbers to match the table, please verify}. 
Although overall performance drops, adding irrelevant context actually increases performance on unanswerable questions. Although retrieval of external knowledge has demonstrated success on other NLP tasks, in our setting, it did not improve performance. We find similar results on \pubmedqa shown in APP.~\ref{app:distractibility}. We also observed that adding more pieces of ambiguous context (Figure~\ref{fig:append_in_paper}) first caused drops in performance before improving performance. Since ambiguous context comes from the same paper, it is not unlikely that some of these passages may provide answers to the question. 

% \noindent\textbf{Distraction effect is highly relevant to answer type} As shown in Figure~\ref{fig:append_in_paper}, abstractive answer is most susceptible to various context. Adding more irrelevant context to questions with abstractive answer can decrease the performance while adding more ambiguous context could improve the performance.

\paragraph{In-context learning with noisy context improves robustness} Adding noisy context in ICL examples consistently and effectively reduces the distractibility of LLMs on \qasper and \pubmedqa. As shown in Figure~\ref{fig:ctx_perturb_gpt}, adding ambiguous or irrelevant context during ICL increases model robustness to most types of noisy context at test time. Similar results on \pubmedqa is included in APP.~\ref{app:distractibility}

% when adding LLM-generated context from 0.41 to 0.50 \lucy{i do not see this in the figure. looks like performance drops for most settings??}.
% {\color{red}In chatgpt, irrelevant context as perturbation works while ambiguous context doesn't work.  In \gpt, both perturbation works.} 

\begin{figure}[t!]
\centering
\includegraphics[width=0.44\textwidth,trim={1cm 0.5cm 1cm 1.3cm},clip]{figure/append_in_paper.pdf}
\caption{F1 change when adding multiple paragraphs of ambiguous context on top of gold context on \qasper using GPT-3.}\label{fig:append_in_paper}
\end{figure}

\begin{figure}[t!]  
\centering
\includegraphics[width=0.44\textwidth,trim={1cm 0.5cm 1cm 1cm},clip]{figure/ctx_perturb_gpt.pdf}
\caption{F1 Performance comparison on \qasper dataset about adding four type of context (ambiguous, irrelevant, wikipedia, generated) on the top of gold context under three ways of demonstrations in ICL (gold context, gold context with irrelevant context, gold context with ambiguous context) using GPT-3. 
}\label{fig:ctx_perturb_gpt}
\end{figure}


% \textbf{{Ablation study}
% \textbf{Paragraph order matters}



\begin{table}[t!]
\small
\centering
\begin{tabular}{lccccc}
\toprule
Context type &  none &  yes & no  & ALL  & ALL_{Macro} \\ 
\midrule
\multicolumn{6}{c}{ChatGPT} \\
\midrule
gold &0.56&0.63 &0.2& \textbf{0.508} &\textbf{0.455}\\
random &0.70&0.43&0.2 & 0.38&0.37 \\ 
From Wikipedia & 0.78 &  0.41 & 0.25 &0.39&0.39  \\
LLM-generated & 0.70& 0.30 & 0.222  &0.376&0.347\\
\midrule
\multicolumn{6}{c}{\gpt} \\
\midrule
gold &0.79&0.68 &0.33& \textbf{0.67} &\textbf{0.58} \\
random &0.59&0.5&0.49& 0.51 &0.49\\ 
From Wikipedia  &  0.41 & 0.25 &0.78& 0.22 &0.22   \\
LLM-generated & 0.12 & 0.29 & 0.48 &0.21& 0.21\\
\bottomrule
\end{tabular}
  \caption{Accuracy performance comparison on \pubmedqa dataset when four types of noisy context are added in addition to gold context under the zero-shot setting. }
\label{tab:dis_context_type_pubmed}
\end{table}




% next experiments:

% 1. in-domain and out of domain
% 2. dataset consists various question type
% 3. entities are too generic and prompt galactica to generate more domain-specific entities. 



% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccccccc}
% \hline
% #&method & shots & docs & extractive & abstractive & boolean & none & answer F1  \\ 
% \hline

%  1& baseline gpt-3.5 &3& 3 & 0.636 & 0.222 & 0.812 & 0.958 & 0.606 \\
%  2&seed =101 gpt-3.5 &3& 3 & 0.580 & 0.203 & 0.806 & 0.967 & 0.587 \\
%  3&seed =17 gpt-3.5 &3& 3 & 0.631 & 0.159 & 0.833 & 0.851 & 0.580 \\


%   4&baseline chatgpt &3&3 &  0.487 & 0.221 & 0.441&  0.916& 0.487 \\
%  5&seed =101  chatgpt &3& 3 &  0.562 & 0.203 & 0.620 & 1.0 & 0.561 \\
%  6&seed =17  chatgpt &3&3 &  0.526 &  0.209 &  0.629& 0.972& 0.544 \\

% \hline
% \end{tabular}
%   \caption{ gold evidence + different prompt}
% \label{tab:filter_four}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{ccccccccc}
% \hline
% method & shots & docs & extractive & abstractive & boolean & none & answer F1  \\ 
% \hline

%  best prompt+best evidence  &3& 3 & 0.636 & 0.222 & 0.812 & 0.958 & 0.606 \\
%  random prompt+best evidence  &3& 3 & 0.631 & 0.159 & 0.833 & 0.851 & 0.580 \\
% best prompt+random evidence &3& 3 &  0.089 &  0.107 & 0.433 &   0.75 &  0.238  \\

% \hline
% \end{tabular}
%   \caption{ gold evidence + different prompt}
% \label{tab:filter_four}
% \end{table*}

% We find that 
% -1.  compared to the baseline, given no context, extractive F1 and abstractive F1 is close to 0. boolean F1 is below random guess. Unanswerable F1 is 1. It indicates that qasper dataset is a highly context-dependent task. 
% -2. compared to the baseline, bad context ? ( paragraphs from other papers) are even worse than no context
% -3.  compared to the baseline, irrelevant context?( paragraphs from the same papers) are even worse than no context
% 1 compared to the baseline,  paragraph order matters.  listing the paragraph in order is better than random order. 
% 2. compared to 1: adding a random paragraph from the other paper, extractive answer's F1 increases but others drops. total F1 i from 0.581 to 0.573.
% 3. compared to baseline, appending a random paragraph from the other paper, extractive performance keeps the same, abstractive decreases, boolean decreases, unanswerable decreases. 
% 4. Compared to 3: Instruction to ignore the irrelevant documents doesn't work. 
% 5. Compared to baseline, appending a random paragraph from the same paper helps. extractive keeps the same, abstraive increases.
% 6. Prompts consists of four question types yields lower performance. Maybe because that the ratio of boolean and unanswerable is much lower than previous ones.
% 7. general domain question answering are less context-dependent than 






% \begin{table*}[t]
% \centering
% \begin{tabular}{cp{0.3\linewidth}cccccccc}
% \hline
% #&method & shots & docs & extractive & abstractive & boolean & none & answer F1  \\ 
% \hline
% -1&no context &0& 0 &  0.003 & 0.013 & 0.414 & 1.0 &  0.238 \\
% -2&random evidence from other paper &3& 3 &  0.019 & 0.025 & 0.316 &  0.9375 &  0.199 \\
% -3&random evidence from the same paper &3& 3 &  0.089 &  0.107 & 0.433 &   0.75 &  0.238  \\
% baseline  & gold evidence  &3& 3 & 0.636 & 0.222 & 0.812 & 0.958 & 0.606  \\
% 1  & gold evidence+random order  &3& 3 &  0.588 & 0.220 & 0.742 & 1.0 & 0.581  \\
% 2&gold + other-paper+random order   &3& 3 & 0.633 &  0.178 & 0.7096 & 0.857 &  0.573\\

% 3&gold + other-paper +append  &3& 3 & 0.635 &  0.209 & 0.727 & 0.884  &  0.581 \\
% 4&gold + other-paper +append +instruct ignore &3& 3 & 0.628 &   0.195 & 0.757 &  0.88  &  0.579 \\

% 5&gold+ in-paper+append  &3& 4 & 0.639 & 0.231 & 0.8 & 0.9 &  0.615 \\

% 6&4prompt &4& 3 & 0.592 & 0.201 & 0.620 & 1.0 & 0.577 \\
% 7& knn prompt &3& 3 & 0.648 & 0.269 &  0.7 & 0.888 & 0.602 \\

% \hline
% \end{tabular}
%   \caption{prompts(given) + golden evidence}
% \label{tab:filter_four}
% \end{table*}





  




% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccccccc}
% \hline
% &method & shots & docs & extractive & abstractive & boolean & none & answer F1 &evidence F1 \\ 
% \hline

% given prompt top_p= 0_1 & gpt-3.5 &3& 3 & 0.648 &   0.232 &  0.875 & 1.0 & 0.632 & 0.917\\
% given prompt top_p= 0_2 & gpt-3.5 &3& 3 & 0.643 &  0.202 & 0.843 & 1.0 & 0.620 & 0.917\\
% 4 prompt top_p= 0_1  & gpt-3.5 &3& 3 & 0.595 & 0.209 & .620 & 1.0 & 0.578 & 0.917\\
%  4 prompt   top_p= 0_2& gpt-3.5  &3&3 & 0.606 & 0.206 & .620 &  1.0&  0.585 & 0.917\\

% \hline
% \end{tabular}
%   \caption{prompts(given) compared with 4 prompts. performance decrease maybe due to the fact the extractive and abstractive questions have high ratios in the dataset. Other types of question as demontrations may hurt the performance.}
% \label{tab:filter_four}
% \end{table*}





% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccccccc}
% \hline
% &method & shots & docs & extractive & abstractive & boolean & none & answer F1 &evidence F1 \\ 
% \hline
% no context top_p= 0_1 & gpt-3.5 &0& 0 & 0.003 & 0.013 &   0.464 & 1.0 & 0.247 & 0.917\\

% given prompt top_p= 0_1 & gpt-3.5 &3& 3 & 0.648 &   0.232 &  0.875 & 1.0 & 0.632 & 0.917\\
% given prompt top_p= 0_2 & gpt-3.5 &3& 3 & 0.643 &  0.202 & 0.843 & 1.0 & 0.620 & 0.917\\
% given prompt+random top_p= 0_1  & gpt-3.5 &3& 3 &  0.646 &  0.232 & 0.793 & 0.903 & 0.621 & 0.917\\
% given prompt+random   top_p= 0_2& gpt-3.5  &3&3 & 0.643 &  0.228 &  0.8 &  0.9 &  0.618 & 0.917\\

% \hline
% \end{tabular}
%   \caption{Based on given prompt top_p = 0, And one paragraph in the same paper but not gold evidence to the context. }
% \label{tab:filter_four}
% \end{table*}





% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccccccc}
% \hline
% &method & shots & docs & extractive & abstractive & boolean & none & answer recall &evidence F1 \\ 
% \hline
% 1& gpt-3.5 &3& 3 &  0.654 & 0.228 & 0.788 & 0.958 &  0.608 & 0.917\\
%  2& chatgpt &3&3 &   0.627 & 0.284 & 0.621 &  1.0 & 0.605 & 0.917\\

% \hline
% \end{tabular}
%   \caption{prompts(given) + golden evidence}
% \label{tab:filter_four}
% \end{table*}




% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccc}
% \hline
% &method & shots & docs & acc & F1  \\ 
% \hline
% 1& gpt-3.5 &3& no context &  0.56 & 0.44 \\
% 1& gpt-3.5 &3& golden evidence &  0.66 & 0.56 \\
%  2& gpt-3.5 &3&generated background &   0.37 & 0.33 \\
% 1& chatgpt &3& no context &  0.23 & 0.20 \\
% 1& chatgpt &3& golden evidence &  0.40 & 0.38 \\

% \hline
% \end{tabular}
%   \caption{pubmed}
% \label{tab:bioasq}
% \end{table*}



% pubmedQA
% chatGPT zero shot context
% Accuracy 0.240000
% Macro-F1 0.204255

% chatGPT zero shot context + generated background
% Accuracy 0.260000
% Macro-F1 0.238721






% galactica zero shot context
% Accuracy 0.634744
% Macro-F1 0.449970


% \begin{table*}[t]
% \centering
% \begin{tabular}{cccccc}
% \hline
% &method & shots & docs & acc & F1  \\ 
% \hline
% 1& gpt-3.5 &3& no context&  0.76 & 0.65 \\
% 1& gpt-3.5 &3&golden evidence &  0.95 & 0.943 \\
%  2& gpt-3.5 &3&generated &   0.74 & 0.70 \\
% 2& chatgpt &3&no context &   0.80 & 0.75 \\
% 2& chatgpt &3&golden evidence &   0.97 & 0.96 \\

% \hline
% \end{tabular}
%   \caption{bioasq}
% \label{tab:bioasq}
% \end{table*}


% 5c2f8127133db5eb78000032
% yes
% no
% 5c58ac2286df2b917400000f
% yes
% no
% 5c674aed7c78d69471000019
% yes
% no
% 5c5839e707647bbc4b00001f
% no
% yes
% 5ca0fa96ecadf2e73f000048
% no
% yes
% 5c9f7bb6ecadf2e73f00003e
% no
% yes
% 5ca5127eecadf2e73f00004c
% no
% yes


==> tables/answer_change_old.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cccc|cccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{SQUAD2}} & \multicolumn{4}{c|}{\textbf{Pubmed}} & \multicolumn{4}{c|}{\textbf{Qasper}} & \multicolumn{4}{c|}{\textbf{BioASQ}} \\
\scriptsize\textbf{Model} & 
\scriptsize Retain(has) & \scriptsize Retain(no) & \scriptsize update & \scriptsize other  & 
\scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
\scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
\scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 \scriptsize LLAMAv2-13B 
  & 1.7 & 12.2 & 66.4 & 22.4
  &17.2 &14.4 &54.8 &13.6
    & 15.6 & 21.1 & 31.2 & 47.7
 & 36.4 & 0.0 &0.7&62.9  \\

 \scriptsize VICUNA1.5-13B 
   & 2.9 & 8.8 &27.7&63.4
& 50.4   &2.4 &39.2 &8.0
 & 26.1 & 6.9 & 16.1& 77.1
    & 69.3 & 0.0 &11.4&19.3
\\

 
 \scriptsize FLAN-XL 
   & 0.0 & 43.7 & 55.9& 0.4
   & 62.8 & 0.0 &0.0&37.2
    & 14.7 & 20.2 &52.3&27.5
 & 71.4 &0.0 & 0.0& 28.6

  \\

 
\scriptsize ChatGPT
   & 52.5 & 21.0 &3.4&75.6
   & 10.8 & 41.2 &43.2&4.8
    & 3.2 & 29.4 & 64.7&6.0
 & 36.4 & 0.0 &0.7&62.9  \\
 
% \scriptsize GPT3 
%   & 36.4 & 0.0 &0.7&62.9
%    & 36.4 & 0.0 &0.7&62.9
%     & 3.2 & 29.4 & 64.7&6.0
%  & 55.0 & 2.1 &22.8&20.0  \\
\bottomrule
\end{tabular}}
\caption{Results for the setting from context to no context across different models and various datasets. \textit{Retain(has)} stands for the model retains to previous answer for the answerable questions and \textit{Retain(no)} for unanswerable questions. \textit{Update} means models change their answer to ``unanswerable''.
\textit{Other} means left senarios. \vspace{-0.25em}}
\label{tab:models}
\end{table*}





==> tables/answerc_change.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cccc|cccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{SQUAD2} (50\% UnAns)} & \multicolumn{4}{c|}{\textbf{Pubmed}} & \multicolumn{4}{c|}{\textbf{Qasper (10\% UnAns)}} & \multicolumn{4}{c|}{\textbf{BioASQ}} \\
\scriptsize\textbf{Model} & 
\scriptsize A \rightarrow A' & \scriptsize A \rightarrow U & \scriptsize U \rightarrow A' & \scriptsize  U \rightarrow U  & 
\scriptsize A \rightarrow A' & \scriptsize A \rightarrow U & \scriptsize U \rightarrow A' & \scriptsize  U \rightarrow U  & 
\scriptsize A \rightarrow A' & \scriptsize A \rightarrow U & \scriptsize U \rightarrow A' & \scriptsize  U \rightarrow U  & 
\scriptsize A \rightarrow A' & \scriptsize A \rightarrow U & \scriptsize U \rightarrow A' & \scriptsize  U \rightarrow U  & 
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 \scriptsize LLAMAv2-13B 
  & 63.9 & 27.7 & 2.52 & 5.88
  &98.5 & 0.0 & 1.5 & 0.0
    & 28.0 & 66.1 & 0.92 & 5.0
 & 100.0 & 0.0 & 0.0 & 0.0  \\

 \scriptsize VICUNA1.5-13B 
   & 39.4 & 41.2 & 4.6 & 14.7
& 99.2   &0.8 &0.0 &0.0
 & 14.7 & 76.6 & 0.0 & 8.72
    & 100.0 & 0.0 & 0.0 &0.0
\\

 
 \scriptsize FLAN-XL 
   & 0.4 & 55.9 & 0.0 & 43.7
   & 100.0 & 0.0 &0.0&0.0
    & 26.6 & 52.3 & 0.9 &20.2
 & 100.0 &0.0 & 0.0& 0.0

  \\

 
\scriptsize ChatGPT
   & 64.7 & 2.9 & 2.5 & 29.8
   & 11.6 & 43.2 &4.0&41.2
    & 4.6 & 64.7 & 1.4& 29.4
 & 51.4 & 48.6 &0.0& 0.0 \\
 
% \scriptsize \gpt 
%   & 36.4 & 0.0 &0.7&62.9
%    & 36.4 & 0.0 &0.7&62.9
%     & 3.2 & 29.4 & 64.7&6.0
%  & 55.0 & 2.1 &22.8&20.0  \\
\bottomrule
\end{tabular}}
\caption{Results for the setting from context to no context($C \rightarrow NC$) across different models and various datasets.  $U$ means the answer is        ``unanswerable''. $A$ refers to any answer other than ``unanswerable'' under with context setting while $A'$ is the same meaning under no context setting. We could see that FLAN-T5-XL perform the best abstention performance among four models in \squad dataset.  }
\label{tab:answer_change}
\end{table*}


% \begin{table*}[t!]
% \centering
% \small
% \resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cccc|cccc|}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{SQUAD2} (50\% UnAns)} & \multicolumn{4}{c|}{\textbf{Pubmed}} & \multicolumn{4}{c|}{\textbf{Qasper (10\% UnAns)}} & \multicolumn{4}{c|}{\textbf{BioASQ}} \\
% \scriptsize\textbf{Model} & 
% \scriptsize A \rightarrow A' & \scriptsize A \rightarrow U & \scriptsize U \rightarrow A' & \scriptsize  U \rightarrow U  & 
% \scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
% \scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
% \scriptsize Retain_has & \scriptsize Retain_no & \scriptsize update & \scriptsize other  & 
% \midrule
% \parbox[t]{1mm}{\multirow{5}{*}} 
%  \scriptsize LLAMAv2-13B 
%   & 1.7 & 12.2 & 66.4 & 22.4
%   &17.2 &14.4 &54.8 &13.6
%     & 15.6 & 21.1 & 31.2 & 47.7
%  & 36.4 & 0.0 &0.7&62.9  \\

%  \scriptsize VICUNA1.5-13B 
%    & 2.9 & 8.8 &27.7&63.4
% & 50.4   &2.4 &39.2 &8.0
%  & 26.1 & 6.9 & 16.1& 77.1
%     & 69.3 & 0.0 &11.4&19.3
% \\

 
%  \scriptsize FLAN-XL 
%    & 0.0 & 43.7 & 55.9& 0.4
%    & 62.8 & 0.0 &0.0&37.2
%     & 14.7 & 20.2 &52.3&27.5
%  & 71.4 &0.0 & 0.0& 28.6

%   \\

 
% \scriptsize ChatGPT
%    & 52.5 & 21.0 &3.4&75.6
%    & 10.8 & 41.2 &43.2&4.8
%     & 3.2 & 29.4 & 64.7&6.0
%  & 36.4 & 0.0 &0.7&62.9  \\
 
% % \scriptsize GPT3 
% %   & 36.4 & 0.0 &0.7&62.9
% %    & 36.4 & 0.0 &0.7&62.9
% %     & 3.2 & 29.4 & 64.7&6.0
% %  & 55.0 & 2.1 &22.8&20.0  \\
% \bottomrule
% \end{tabular}}
% \caption{Results for the setting from context to no context across different models and various datasets. \textit{Retain(has)} stands for the model retains to previous answer for the answerable questions and \textit{Retain(no)} for unanswerable questions. \textit{Update} means models change their answer to ``unanswerable''.
% \textit{Other} means left senarios. }
% \label{tab:answer_change}
% \end{table*}

==> tables/baseline.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|c|cc|cc|cc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{\textbf{SQUAD2}} & \multicolumn{2}{c|}{\textbf{Pubmed}}  & \multicolumn{2}{c|}{\textbf{BioASQ}} & \multicolumn{2}{c|}{\textbf{Qasper}} \\
\scriptsize\textbf{Model} & 
\scriptsize Constrained &  
\scriptsize Constrained & \scriptsize Free-form & \scriptsize Constrained & \scriptsize Free-form 
& \scriptsize Constrained   & \scriptsize Free-form \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 \scriptsize LLAMAv2-13B & 
 \baseline{55.4} &  
 
 \baseline{51.2} &  \midpointgradientcell{-41.0}{-36.1}{6.7}{0}{neg}{pos}{\opacity}{0} &

  \baseline{98.4} & \midpointgradientcell{-18.0}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0}  &
  
 \baseline{45.6} &  &
 

 \scriptsize VICUNA1.5-13B & 
 \baseline{60.9} & 
 
 \baseline{48.6} & &

  \baseline{94.3} & \midpointgradientcell{-19.0}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
  
 \baseline{54.0} & &
 

 
 \scriptsize FLAN-XL & 
 \baseline{78.6} & 
 
 \baseline{38.0} & &


  \baseline{86.0} & &
  
 \baseline{46.6} & &
 

 
\scriptsize ChatGPT& 
 \baseline{64.5} &  
 
 \baseline{58.8} &  & 

 \baseline{97.6} & \midpointgradientcell{-0.4}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &

 
 \baseline{54.4} &  & 

 
% \scriptsize GPT3 & 
%  \baseline{38.4} & \midpointgradientcell{6.6}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{53.6} & \midpointgradientcell{-53.6}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{7.1}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{34.9} & \midpointgradientcell{-7.1}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{1.6}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{63.5} & \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} \\
\bottomrule
\end{tabular}}
\caption{Results for the zero-shot performance across different models and different datasets.}
\label{tab:baseline}
\end{table*}



==> tables/baseline_constrained.tex <==
\begin{table}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|c|c|c|c|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{\textbf{SQUAD2}} & \multicolumn{1}{c|}{\textbf{Pubmed}}  & \multicolumn{1}{c|}{\textbf{BioASQ}} & \multicolumn{1}{c|}{\textbf{Qasper}} \\
\scriptsize\textbf{Model} & 
\scriptsize Constrained &  
\scriptsize Constrained & \scriptsize Constrained &  \scriptsize Constrained   \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 \scriptsize LLAMAv2-13B & 
 55.4 &  
 
51.2 &  

98.4 &
  
45.6 &  

 \scriptsize VICUNA1.5-13B & 
60.9 & 
 
48.6 & 

94.3 & 
  
54.0 & 
 
 \scriptsize FLAN-XL & 
78.6 & 
 38.0 & 
86.0 & 
46.6 & 
 

\scriptsize ChatGPT& 
61.0 &  
 
58.8 &  

97.6 &

54.4  & 

 
% \scriptsize GPT3 & 
%  \baseline{38.4} & \midpointgradientcell{6.6}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{53.6} & \midpointgradientcell{-53.6}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{7.1}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{34.9} & \midpointgradientcell{-7.1}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{1.6}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&\midpointgradientcell{3.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
%  \baseline{63.5} & \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} \\
\bottomrule
\end{tabular}}
\caption{Results for the zero-shot performance across different models and different datasets.}
\label{tab:baseline_constrained}
\end{table}



==> tables/model_answerability.tex <==



\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccccc|cccccc|ccc|cccccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c|}{\textbf{
SQUAD2}} & \multicolumn{6}{c}{\textbf{Pubmed}} & \multicolumn{3}{c}{\textbf{BioASQ}} & \multicolumn{6}{c}{\textbf{Qasper}} \\
\midrule
\multicolumn{1}{c}{}  & \multicolumn{3}{c|}{\textbf{
Answerable}} & \multicolumn{3}{c|}{\textbf{
Unanswerable}} & \multicolumn{3}{c|}{\textbf{
Answerable}} & \multicolumn{3}{c|}{\textbf{
Unanswerable}} & \multicolumn{3}{c|}{\textbf{
Answerable}} & \multicolumn{3}{c|}{\textbf{
Answerable}} & \multicolumn{3}{c|}{\textbf{
Unanswerable}} \\
\midrule
\scriptsize\textbf{Model} & \scriptsize Base & \scriptsize NC & \scriptsize RC  & \scriptsize Base & \scriptsize NC & \scriptsize RC & \scriptsize Base & \scriptsize NC & \scriptsize RC & \scriptsize Base & \scriptsize NC & \scriptsize RC  & \scriptsize Base & \scriptsize NC & \scriptsize RC& \scriptsize Base & \scriptsize NC & \scriptsize RC  & \scriptsize Base & \scriptsize NC & \scriptsize RC\\
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 
 LLAMAv2-13B & 
 %squad2
 \baseline{1.68} & 
 \midpointgradientcell{18.4}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{78.1}{-5.5}{24.1}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{15.1} & 
 \midpointgradientcell{32}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{67.3}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0} & 

 %pubmed
 \baseline{0.9} & \midpointgradientcell{0.0}{-4.6}{54.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-7.5}{10.8}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{3.7} & 
 \midpointgradientcell{0.0}{-4.6}{54.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{0.0}{-7.5}{10.8}{0}{neg}{pos}{\opacity}{0} & 
 

 %bioasq
 \baseline{0.0} & \midpointgradientcell{0.0}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} &

 %qasper
  \baseline{3.0} & \midpointgradientcell{ 66.0 }{-8.9}{32.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{19.5 }{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} &

   \baseline{41.1} & 
 \midpointgradientcell{ 41.2}{-8.9}{62.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{ 7}{-8.3}{30.9}{0}{neg}{pos}{\opacity}{0}


\\

 VICUNA1.5-13B &
 %squad2
  \baseline{5.88} & \midpointgradientcell{43.7}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{89.9}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} & 

  \baseline{32.8} & 
  \midpointgradientcell{29.4}{-6.1}{46.7}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{61.3}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} & 

%pubmed
 \baseline{0.0} & \midpointgradientcell{0.9}{-4.6}{40.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} &
 
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-4.6}{40.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} &

 
%bioasq
 \baseline{0.0} & \midpointgradientcell{0.0}{-8.9}{12.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&

 %qasper
  \baseline{4.1} & \midpointgradientcell{80}{-8.9}{52.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{13.1}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
  
 \baseline{44.1} & 
 \midpointgradientcell{46.4}{-8.9}{32.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{ -5.6}{-8.3}{20.9}{0}{neg}{pos}{\opacity}{0}
    
    \\
 
 FLAN-XL & 
 %squad2
  \baseline{6.7} & 
  \midpointgradientcell{90.3}{-6.1}{36.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{90.8}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} & 
 
  \baseline{80.7} & 
  \midpointgradientcell{19.3}{-6.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{19.3}{-5.5}{16.7}{0}{neg}{pos}{\opacity}{0} &
 

 
 
 %pubmed
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&

 \baseline{0.0} & \midpointgradientcell{0.0}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 
 
%bioasq
  \baseline{0.0} & \midpointgradientcell{0.0}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 

 
 %qasper
  \baseline{25.9} & \midpointgradientcell{54.2}{-8.9}{62.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{43.0}{-8.3}{50.9}{0}{neg}{pos}{\opacity}{0} &

 \baseline{89.6} & 
 \midpointgradientcell{3.5}{-8.9}{72.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{4.6}{-8.3}{70.9}{0}{neg}{pos}{\opacity}{0}
  
  \\
 
ChatGPT& 
%squad2
 \baseline{27.9} & 
 \midpointgradientcell{72.1}{-6.1}{32}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{72.0}{-5.5}{32}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{56.3} &
 \midpointgradientcell{40.5}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{43.6}{-5.5}{24.1}{0}{neg}{pos}{\opacity}{0} & 
 
 %pubmed
 \baseline{43.9} & 
 \midpointgradientcell{40.0}{-4.6}{34.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{5.8}{-7.5}{11.8}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{55.6} & 
 \midpointgradientcell{33.3}{-4.6}{24.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-7.5}{31.8}{0}{neg}{pos}{\opacity}{0} &



%bioasq
 \baseline{0.0} &
 \midpointgradientcell{48.6}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-5.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
 
 %qasper
  \baseline{30.7} & \midpointgradientcell{32.6}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} &

 \baseline{100.0} & 
 \midpointgradientcell{0.0}{-8.9}{72.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}
  
 \\
 
% \gpt & 
% %squad2
%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


%  %pubmed
%  \baseline{14.4} & 
%  \midpointgradientcell{-9.7}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{2.1} & 
%  \midpointgradientcell{20.8}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
 
%  %qasper
%   \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}

%     \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\

\bottomrule
\end{tabular}}
\caption{Results for the abstention ability across different models. \textit{NC} stands for no context and \textit{RC} for random context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with gold context}. Notice that models with higher base scores are better at abstaining.}  
\label{tab:ans_base}
\end{table*}

==> tables/model_unanserability.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccc|ccc|ccc|ccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c|}{\textbf{
SQUAD2}} & \multicolumn{3}{c}{\textbf{Pubmed}} & \multicolumn{3}{c}{\textbf{Qasper}} \\
\scriptsize\textbf{Model} & \scriptsize Base & \scriptsize NC & \scriptsize RC  & \scriptsize Base & \scriptsize NC & \scriptsize RC & \scriptsize Base & \scriptsize NC & \scriptsize RC \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 LLAMAv2-13B & 
 %squad
 \baseline{15.1} & 
 \midpointgradientcell{32}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{67.3}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0} & 
 

 %pubmed
 \baseline{3.7} & 
 \midpointgradientcell{0.0}{-4.6}{54.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{0.0}{-7.5}{10.8}{0}{neg}{pos}{\opacity}{0} & 

 %qasper
 \baseline{41.1} & 
 \midpointgradientcell{ 41.2}{-8.9}{62.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{ 7}{-8.3}{30.9}{0}{neg}{pos}{\opacity}{0} \\
 

 VICUNA1.5-13B & 
%squad
  \baseline{32.8} & 
  \midpointgradientcell{29.4}{-6.1}{46.7}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{61.3}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} & 

  %pubmed
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-4.6}{40.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} &

 %qasper
 \baseline{44.1} & 
 \midpointgradientcell{46.4}{-8.9}{32.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{ -5.6}{-8.3}{20.9}{0}{neg}{pos}{\opacity}{0}\\


 
 FLAN-XL & 
 %squad
  \baseline{80.7} & 
  \midpointgradientcell{19.3}{-6.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{19.3}{-5.5}{16.7}{0}{neg}{pos}{\opacity}{0} &
  
 \baseline{0.0} & \midpointgradientcell{0.0}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{0.0}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{89.6} & 
 \midpointgradientcell{3.5}{-8.9}{72.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{-1}{-8.3}{70.9}{0}{neg}{pos}{\opacity}{0} \\
 

ChatGPT& 
%squad
 \baseline{56.3} &
 \midpointgradientcell{40.5}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
 %pubmed
 \baseline{55.6} & 
 \midpointgradientcell{33.3}{-4.6}{24.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-7.5}{31.8}{0}{neg}{pos}{\opacity}{0} &
 %qasper
 \baseline{100.0} & 
 \midpointgradientcell{0.0}{-8.9}{72.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\
 
\gpt & 
%squad
 \baseline{63.9} & 
 \midpointgradientcell{35.3}{-6.1}{26.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
 %pubmed
 \baseline{25.9} & 
 \midpointgradientcell{33.4}{-4.6}{24.8}{0}{neg}{pos}{\opacity}{0} & 
 \midpointgradientcell{}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 
 %qasper
 \baseline{96.7} &
 \midpointgradientcell{-7.2}{-8.9}{62.8}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\
 
\bottomrule
\end{tabular}}
\caption{Results for the abstention ability across different models for \textbf{unanswerable questions} in various datasets. \textit{NC} stands for no context and \textit{RC} for random context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with gold context}. Notice that models with higher base scores are better at abstaining.     }
\label{tab:unans_base}
\end{table*}

==> tables/no_context.tex <==



\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cc|cccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{
SQUAD2}} & \multicolumn{4}{c}{\textbf{Pubmed}} & \multicolumn{2}{c}{\textbf{BioASQ}} & \multicolumn{4}{c}{\textbf{Qasper}} \\
\midrule
\multicolumn{1}{c}{}  & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} \\
\midrule
\scriptsize\textbf{Model} & \scriptsize Base & \scriptsize NC  & \scriptsize Base & \scriptsize NC  & \scriptsize Base & \scriptsize NC & \scriptsize Base & \scriptsize NC  & \scriptsize Base & \scriptsize NC & \scriptsize Base & \scriptsize NC  & \scriptsize Base & \scriptsize NC \\
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 
 LLAMAv2-13B & 
 %squad2
 \baseline{14.3} & 
 \midpointgradientcell{10.7}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &

 \baseline{58.5} & 
 \midpointgradientcell{-22.4}{-22.4}{87.4}{0}{neg}{pos}{\opacity}{0} &


 %pubmed
 \baseline{6.3} & 
 \midpointgradientcell{12.1}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{9.1} & 
 \midpointgradientcell{14.5}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} & 

 

 %bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0}& 

 %qasper
  \baseline{2.7} & \midpointgradientcell{18.5}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} &
  
   \baseline{36.5} & 
 \midpointgradientcell{0.9}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} &


 VICUNA1.5-13B &
 %squad2
  \baseline{20.7} & \midpointgradientcell{14.4}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &

  \baseline{64.7} & 
  \midpointgradientcell{ -21.8}{-22.4}{87.4}{0}{neg}{pos}{\opacity}{0} &

%pubmed
 \baseline{62.5} & \midpointgradientcell{25.8}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} &
 
 \baseline{60.0} & 
 \midpointgradientcell{27.3}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} & 


 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 10.7}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{29.3} & \midpointgradientcell{ 39.0}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 
  
 \baseline{57.0} & 
 \midpointgradientcell{20.7}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} &



 FLAN-XL & 
 %squad2
  \baseline{4.7} & 
  \midpointgradientcell{87.4}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &
 
  \baseline{84.5} & 
  \midpointgradientcell{10.3}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &

 

 
 
 %pubmed
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{0.0} & \midpointgradientcell{0.0}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} & 
 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0}&  
 
 %qasper
  \baseline{8.0} & \midpointgradientcell{50.1}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{74.1} & 
 \midpointgradientcell{0.5}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 

  

 
ChatGPT& 
%squad2
 \baseline{3.7} & 
 \midpointgradientcell{36.4}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &

 \baseline{53.3} &
 \midpointgradientcell{2.8}{-6.1}{87.4}{0}{neg}{pos}{\opacity}{0} &

 
 %pubmed
 \baseline{26.3} & 
 \midpointgradientcell{43.4}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{27.3} & 
 \midpointgradientcell{32.7}{-4.6}{87.4}{0}{neg}{pos}{\opacity}{0} &



%bioasq

 \baseline{0.0} & \midpointgradientcell{ 35.7 }{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{16.2} & \midpointgradientcell{3.9}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{91.7} & 
 \midpointgradientcell{3.1}{-8.9}{87.4}{0}{neg}{pos}{\opacity}{0} & 

  

 
% \gpt & 
% %squad2
%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


%  %pubmed
%  \baseline{14.4} & 
%  \midpointgradientcell{-9.7}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{2.1} & 
%  \midpointgradientcell{20.8}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
 
%  %qasper
%   \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}

%     \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\

\bottomrule
\end{tabular}}
\caption{Results for the abstention ability across different models for \textbf{answerable questions} 
 and \textbf{unanswerable questions} in various datasets. \textit{NC} for no context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with given context}. Notice that models with higher base scores are better at abstaining. }  
\label{tab:no_context}
\end{table*}

==> tables/noisy_context.tex <==



\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cc|cccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{
SQUAD2}} & \multicolumn{4}{c}{\textbf{Pubmed}} & \multicolumn{2}{c}{\textbf{BioASQ}} & \multicolumn{4}{c}{\textbf{Qasper}} \\
\midrule
\multicolumn{1}{c}{}  & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} \\
\midrule
\scriptsize\textbf{Model} & \scriptsize Base & \scriptsize NC*  & \scriptsize Base & \scriptsize NC*  & \scriptsize Base & \scriptsize NC* & \scriptsize Base & \scriptsize NC*  & \scriptsize Base & \scriptsize NC* & \scriptsize Base & \scriptsize NC*  & \scriptsize Base & \scriptsize NC* \\
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 

 LLAMAv2-13B & 
 %squad2
 \baseline{14.3} & 
 \midpointgradientcell{-10.8}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

 \baseline{58.5} & 
 \midpointgradientcell{-34.6}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &


 %pubmed
 \baseline{6.3} & 
 \midpointgradientcell{48.5}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{9.1} & 
 \midpointgradientcell{54.5}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 

 

 %bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0}& 

 %qasper
  \baseline{2.7} & \midpointgradientcell{21.2 }{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &
  
   \baseline{36.5} & 
 \midpointgradientcell{31.8}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &


 VICUNA1.5-13B &
 %squad2
  \baseline{20.7} & \midpointgradientcell{3.8}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

  \baseline{64.7} & 
  \midpointgradientcell{-6.7}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

%pubmed
 \baseline{62.5} & \midpointgradientcell{3.1}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &
 
 \baseline{60.0} & 
 \midpointgradientcell{10.9}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 


 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{29.3} & \midpointgradientcell{ -1.6}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 
  
 \baseline{57.0} & 
 \midpointgradientcell{36.2}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &



 FLAN-XL & 
 %squad2
  \baseline{4.7} & 
  \midpointgradientcell{-1.7}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &
 
  \baseline{84.5} & 
  \midpointgradientcell{-1.9}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

 

 
 
 %pubmed
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{0.0} & \midpointgradientcell{0.0}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 
 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0}&  
 
 %qasper
  \baseline{8.0} & \midpointgradientcell{-1.2}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{74.1} & 
 \midpointgradientcell{-4.4}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 

  

 
ChatGPT& 
%squad2
 \baseline{3.7} & 
 \midpointgradientcell{1.7}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

 \baseline{53.2} &
 \midpointgradientcell{-2.2}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &

 
 %pubmed
 \baseline{26.3} & 
 \midpointgradientcell{2.9}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{27.3} & 
 \midpointgradientcell{-3.7}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} &



%bioasq

 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{16.2} & \midpointgradientcell{4.8}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{91.7} & 
 \midpointgradientcell{3.5}{-34.6}{54.5}{0}{neg}{pos}{\opacity}{0} & 


 
% \gpt & 
% %squad2
%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


%  %pubmed
%  \baseline{14.4} & 
%  \midpointgradientcell{-9.7}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{2.1} & 
%  \midpointgradientcell{20.8}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
 
%  %qasper
%   \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}

%     \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\

\bottomrule
\end{tabular}}
\caption{Results for the abstention ability across different models for \textbf{answerable questions} 
 and \textbf{unanswerable questions} in various datasets. \textit{We find providing noisy context to \bioasq dataset makes all models fail to abstain.} \textit{NC*} for noisy context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with given context}. Notice that models with higher base scores are better at abstaining.}  
\label{tab:noisy_context}
\end{table*}




==> tables/pubmed_context.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|ccccc|ccccc|ccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c|}{\textbf{\chatgpt}} & \multicolumn{5}{c|}{\textbf{\gpt}} & \multicolumn{5}{c|}{\textbf{LLamaV2}}  \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen & \scriptsize Given & \scriptsize +Giv & \scriptsize +Rand & \scriptsize +Wiki  & \scriptsize +Gen & \scriptsize Given & \scriptsize +Giv  & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen \\
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 
 \scriptsize All& 
  %chatgpt
 \baseline{45.1} & 
 \midpointgradientcell{13.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-6.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{-16.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

%\gpt
 \baseline{67.2} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-16}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-45}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-43}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &


%llama
 \baseline{33.2} & 
 \midpointgradientcell{8.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.5}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-9.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{-13.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
  \\

 \scriptsize None& 
 %chatgpt
 \baseline{56.2} & 
 \midpointgradientcell{-4.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{14.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{22.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{14.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}&

%gpt3
 \baseline{79.1} & 
 \midpointgradientcell{}{-6.1}{56.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.3}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-38.0}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{-67.1}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0}&


%llama
 \baseline{59.3} & 
 \midpointgradientcell{22.1}{-6.1}{10.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{14.8}{-5.5}{10.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{22.2}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{29.6}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}
  \\

\scriptsize Yes&  
%chatgpt
 \baseline{63.3} & 
 \midpointgradientcell{-1.0}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.2}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-22.1}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{-33.1}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

%gpt3
 \baseline{68.2} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-18.3}{-15.5}{64.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-43.1}{-15.5}{54.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{-39.2}{-15.5}{54.1}{0}{neg}{pos}{\opacity}{0}&


%llama
 \baseline{31.9} & 
 \midpointgradientcell{13.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-12.3}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.3}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}

  \\

  \scriptsize No&  
  %\chatgpt
 \baseline{20.3} & 
 \midpointgradientcell{33.2}{-6.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{5.1}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-12.1}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&

%gpt3
 \baseline{33.2} & 
 \midpointgradientcell{}{-6.1}{36.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{16.4}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{45.3}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0}&
\midpointgradientcell{16.1}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{27.1} & 
 \midpointgradientcell{1.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-15.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{-15.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}

  \\
\bottomrule
\end{tabular}}
\caption{Results for the Accuracy performance across different models and various question types on \pubmedqa dataset. }
\label{tab:pubmed}
\end{table*}




==> tables/pubmed_context_new.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c|}{\textbf{\llama}}
& \multicolumn{3}{c|}{\textbf{\vicuna}}
& \multicolumn{3}{c|}{\textbf{\flan}}
& \multicolumn{3}{c|}{\textbf{\chatgpt}}    \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Rand & \scriptsize Given & \scriptsize +Giv & \scriptsize +Rand  & \scriptsize Given & \scriptsize +Giv  & \scriptsize +Rand 
& \scriptsize Given & \scriptsize +Giv  & \scriptsize +Rand &
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 
 \scriptsize All& 
 
%llama
 \baseline{33.2} & 
 \midpointgradientcell{8.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.5}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-9.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 %  \midpointgradientcell{-13.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}
 
%vicuna
 \baseline{52.4} & 
 \midpointgradientcell{2.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.5}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

 %flan
 \baseline{38.2} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-2.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 
 %chatgpt
  \baseline{55.4} & 
 \midpointgradientcell{1.3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{-6.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 %  \midpointgradientcell{-16.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

% %\gpt
%  \baseline{67.2} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-16}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-45}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0}&
%  \midpointgradientcell{-43}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &



  \\

 \scriptsize None& 

%llama
 \baseline{59.3} & 
 \midpointgradientcell{22.1}{-6.1}{10.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{14.8}{-5.5}{10.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{22.2}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
 %  \midpointgradientcell{29.6}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}

%vicuna
 \baseline{48.1} & 
 \midpointgradientcell{-7.4}{-6.1}{10.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{14.8}{-5.5}{10.1}{0}{neg}{pos}{\opacity}{0} &

 %flan
 \baseline{0.0} & 
 \midpointgradientcell{0.0}{-6.1}{10.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.0}{-5.5}{10.1}{0}{neg}{pos}{\opacity}{0} &


 %chatgpt
 \baseline{63.0} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{14.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{22.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}&
 %  \midpointgradientcell{14.0}{-5.5}{14.1}{0}{neg}{pos}{\opacity}{0}&

% %gpt3
%  \baseline{79.1} & 
%  \midpointgradientcell{}{-6.1}{56.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-20.3}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-38.0}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0}&
%   \midpointgradientcell{-67.1}{-5.5}{54.1}{0}{neg}{pos}{\opacity}{0}&



  \\

\scriptsize Yes&  


%llama
 \baseline{31.9} & 
 \midpointgradientcell{13.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-12.3}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-20.3}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}

%vicuna
 \baseline{60.1} & 
 \midpointgradientcell{7.3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

 %flan
 \baseline{98.6} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

 
%chatgpt
 \baseline{62.3} & 
 \midpointgradientcell{-1.0}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.2}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{-22.1}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 %  \midpointgradientcell{-33.1}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

% %gpt3
%  \baseline{68.2} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-18.3}{-15.5}{64.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-43.1}{-15.5}{54.1}{0}{neg}{pos}{\opacity}{0}&
%   \midpointgradientcell{-39.2}{-15.5}{54.1}{0}{neg}{pos}{\opacity}{0}&

  \\

  \scriptsize No&  

%llama
 \baseline{27.1} & 
 \midpointgradientcell{1.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-15.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 %  \midpointgradientcell{-15.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}
 
%vicuna
 \baseline{58.8} & 
 \midpointgradientcell{-3.5}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

  
%flan
 \baseline{25.9} & 
 \midpointgradientcell{0.0}{-6.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{9.5}{-5.5}{10.1}{0}{neg}{pos}{\opacity}{0} &
  
  %\chatgpt
 \baseline{54.1} & 
 \midpointgradientcell{-4.7}{-6.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{5.1}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{-12.1}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&

% %gpt3
%  \baseline{33.2} & 
%  \midpointgradientcell{}{-6.1}{36.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{16.4}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{45.3}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0}&
% \midpointgradientcell{16.1}{-5.5}{34.1}{0}{neg}{pos}{\opacity}{0} &
  \\
\bottomrule
\end{tabular}}
\caption{Results for the Accuracy performance across different models and various question types on \pubmedqa dataset. }
\label{tab:pubmed_context_new}
\end{table*}




==> tables/qasper_context.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|cccccc|cccccc|cccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c|}{\textbf{ChatGPT}} & \multicolumn{6}{c|}{\textbf{\gpt}} & \multicolumn{6}{c|}{\textbf{LLamaV2}}  \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen &\scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand & \scriptsize +Wiki  & \scriptsize +Gen & \scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen \\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 

 \scriptsize All& 
 %chatgpt
 \baseline{57.1} & 
 \midpointgradientcell{4.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{1.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-2.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-10}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-16}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
%gpt3
 \baseline{63.1} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-10.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-22.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{42.4} & 
 \midpointgradientcell{-2.2}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-5.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-8.6}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}   \\

 \scriptsize None& 
 %chatgpt
 \baseline{97.1} & 
 \midpointgradientcell{-0.3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-8.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{2.9}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-5.8}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-11.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 
%gpt3
 \baseline{85.1} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{11.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{0.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.0}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{60.0} & 
 \midpointgradientcell{-5.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.9}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-12.5}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-9.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}   
 \\

 \scriptsize Ext. & 
 %chatgpt
 \baseline{56.1} & 
 \midpointgradientcell{9.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{5.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-0.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-12}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-15.8}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


 %gpt3
 \baseline{65.0} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-10}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-26}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{48.9} & 
 \midpointgradientcell{-5.8}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-11.5}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-8.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-11.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}  
 
 \\

 \scriptsize Abs. & 
 %chatgpt
 \baseline{29.2} & 
 \midpointgradientcell{-3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-9}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-17}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


 %gpt3
 \baseline{37.3} & 
 \midpointgradientcell{}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-15}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-17}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{21.0} & 
 \midpointgradientcell{1.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{1.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-1.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 

  \\
 
\scriptsize Bool.& 
 %chatgpt
 \baseline{69.3} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-23}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-33}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


 %gpt3
 \baseline{77.1} & 
 \midpointgradientcell{}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-25}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

%llama
 \baseline{43.1} & 
 \midpointgradientcell{5.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-12}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.9}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{-10.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
  \\

\bottomrule
\end{tabular}}
\caption{Results for the F1 performance across different models and various question types on qasper dataset. \textit{Given} shows the baseline performance with given context. \textit{+Giv} means that appending one paragraph which is randomly chosen from given context as fair comparison. \textit{+Rand} stands for adding random context on the top of given context. \textit{+WIKI} means adding wikipedia context retrieved by retriever model.  \textit{+Gen} refers to add generated context by ChatGPT.  Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with Given context}. Notice that models with higher base scores are generally less benefit or harmed from the external context.\vspace{-0.25em} \lucy{these models don't match the models discussed in the modeling section}}
\label{tab:models}
\end{table*}




==> tables/qasper_context_new.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|cccc|cccc|cccc|cccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{\llama}}& \multicolumn{4}{c|}{\textbf{\vicuna}}& \multicolumn{4}{c|}{\textbf{\flan}}& \multicolumn{4}{c|}{\textbf{\chatgpt}}   \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand &\scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand &  \scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand &
\scriptsize Given & \scriptsize +Giv & \scriptsize +Abst & \scriptsize +Rand\\
\midrule
\parbox[t]{1mm}{\multirow{5}{*}} 
 \scriptsize All& 

 %llama
 \baseline{42.4} & 
 \midpointgradientcell{-2.2}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-5.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&


  %vicuna
 \baseline{48.5} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-5.5}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

 
   %FLAN
 \baseline{52.9} & 
 \midpointgradientcell{-12.1}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-29.4}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-24.8}{-15.5}{44.1}{0}{neg}{pos}{\opacity}{0}&

 
 %chatgpt
 \baseline{57.1} & 
 \midpointgradientcell{4.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{1.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-2.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}
\\
% %gpt3
%  \baseline{63.1} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-7.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
%  \midpointgradientcell{-10.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-22.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &



 \scriptsize None& 

 %llama
 \baseline{60.0} & 
 \midpointgradientcell{-5.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.9}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-12.5}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&


  %vicuna
 \baseline{39.1} & 
 \midpointgradientcell{6.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{20}{-5.5}{24.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{19.2}{-5.5}{24.1}{0}{neg}{pos}{\opacity}{0}&


  %flan
 \baseline{90.0} & 
 \midpointgradientcell{-0.8}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.5}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{4.6}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&

 
 %chatgpt
 \baseline{97.1} & 
 \midpointgradientcell{-0.3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-8.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{2.9}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}

% %gpt3
%  \baseline{85.1} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{11.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
%  \midpointgradientcell{0.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{-4.0}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &


 \\



 \scriptsize Ext. & 


 %llama
 \baseline{48.9} & 
 \midpointgradientcell{-5.8}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-11.5}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-8.8}{-5.5}{44.1}{0}{neg}{pos}{\opacity}{0}&



  %vicuna
 \baseline{53.2} & 
 \midpointgradientcell{2.8}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-11.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-5.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


%flan
 \baseline{52.8} & 
 \midpointgradientcell{-17.2}{-26.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-40}{-25.5}{44.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-38.2}{-25.5}{44.1}{0}{neg}{pos}{\opacity}{0}&

 
 %chatgpt
 \baseline{56.1} & 
 \midpointgradientcell{9.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{5.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-0.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}



 % %gpt3
 % \baseline{65.0} & 
 % \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-10}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{-13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-26}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &


 
 \\

 \scriptsize Abs. & 
%llama
 \baseline{21.0} & 
 \midpointgradientcell{1.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{1.2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


 %vicuna
 \baseline{29.5} & 
 \midpointgradientcell{-2.8}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.8}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


 %flan
 \baseline{12.5} & 
 \midpointgradientcell{-0.2}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.8}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-8.7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


 
 %chatgpt
 \baseline{29.2} & 
 \midpointgradientcell{-3}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}


 % %gpt3
 % \baseline{37.3} & 
 % \midpointgradientcell{}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{-15}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-17}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &


 

  \\
 
\scriptsize Bool.& 

%llama
 \baseline{43.1} & 
 \midpointgradientcell{5.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-12}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-1.9}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


 %vicuna
 \baseline{71.0} & 
 \midpointgradientcell{-16.2}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-9.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-10.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&

 
 
 %flan
 \baseline{67.6} & 
 \midpointgradientcell{-58.6}{-36.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-53.5}{-35.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-52.3}{-35.5}{4.1}{0}{neg}{pos}{\opacity}{0}&


 %chatgpt
 \baseline{69.3} & 
 \midpointgradientcell{0.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{13}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}


 % %gpt3
 % \baseline{77.1} & 
 % \midpointgradientcell{}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-7}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{2}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 % \midpointgradientcell{-25}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &


  \\

\bottomrule
\end{tabular}}
\caption{Results for the F1 performance across different models and various question types on qasper dataset. \textit{Given} shows the baseline performance with given context. \textit{+Giv} means that appending one paragraph which is randomly chosen from given context as fair comparison. \textit{+Rand} stands for adding random context on the top of given context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with Given context}. Notice that models with higher base scores are generally less benefit or harmed from the external context.\vspace{-0.25em}}
\label{tab:qasper_context_new}
\end{table*}




==> tables/random_context.tex <==



\begin{table*}[t!]
\centering
\small
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cc|cccc|}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c|}{\textbf{
SQUAD2}} & \multicolumn{4}{c}{\textbf{Pubmed}} & \multicolumn{2}{c}{\textbf{BioASQ}} & \multicolumn{4}{c}{\textbf{Qasper}} \\
\midrule
\multicolumn{1}{c}{}  & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Answerable}} & \multicolumn{2}{c|}{\textbf{
Unanswerable}} \\
\midrule
\scriptsize\textbf{Model} & \scriptsize Base & \scriptsize RC  & \scriptsize Base & \scriptsize RC  & \scriptsize Base & \scriptsize RC & \scriptsize Base & \scriptsize RC  & \scriptsize Base & \scriptsize RC & \scriptsize Base & \scriptsize RC  & \scriptsize Base & \scriptsize RC \\
\midrule
\parbox[t]{1mm}{\multirow{4}{*}} 
 LLAMAv2-13B & 
 %squad2
 \baseline{14.3} & 
 \midpointgradientcell{69.3}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

 \baseline{58.5} & 
 \midpointgradientcell{18.6}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &


 %pubmed
 \baseline{6.3} & 
 \midpointgradientcell{87}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{9.1} & 
 \midpointgradientcell{80}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} & 

 

 %bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0}& 

 %qasper
  \baseline{2.7} & \midpointgradientcell{30.3 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} &
  
   \baseline{36.5} & 
 \midpointgradientcell{30.8}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} &


 VICUNA1.5-13B &
 %squad2
  \baseline{20.7} & \midpointgradientcell{71.4}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

  \baseline{64.7} & 
  \midpointgradientcell{29.2}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

%pubmed
 \baseline{62.5} & \midpointgradientcell{36.8}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} &
 
 \baseline{60.0} & 
 \midpointgradientcell{38.2}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} & 


 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{29.3} & \midpointgradientcell{ 46.3}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 
  
 \baseline{57.0} & 
 \midpointgradientcell{37.2}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} &



 FLAN-XL & 
 %squad2
  \baseline{4.7} & 
  \midpointgradientcell{95.2}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &
 
  \baseline{84.5} & 
  \midpointgradientcell{15.5}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

 

 
 
 %pubmed
 \baseline{0.0} & 
 \midpointgradientcell{69.7}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{0.0} & \midpointgradientcell{65.5}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} & 
 
%bioasq
 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0}&  
 
 %qasper
  \baseline{8.0} & \midpointgradientcell{50.1}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{74.1} & 
 \midpointgradientcell{0.5}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 

  

 
ChatGPT& 
%squad2
 \baseline{3.7} & 
 \midpointgradientcell{95.5}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

 \baseline{53.2} &
 \midpointgradientcell{46.3}{-6.1}{95.5}{0}{neg}{pos}{\opacity}{0} &

 
 %pubmed
 \baseline{26.3} & 
 \midpointgradientcell{73.5}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} & 
 
 \baseline{27.3} & 
 \midpointgradientcell{70.9}{-4.6}{95.5}{0}{neg}{pos}{\opacity}{0} &



%bioasq

 \baseline{0.0} & \midpointgradientcell{ 0.0 }{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0}& 
 
 %qasper
  \baseline{16.2} & \midpointgradientcell{68.4}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 

 \baseline{91.7} & 
 \midpointgradientcell{4.1}{-8.9}{95.5}{0}{neg}{pos}{\opacity}{0} & 

  

 
% \gpt & 
% %squad2
%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{30.4} & 
%  \midpointgradientcell{66.4}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &\midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 


%  %pubmed
%  \baseline{14.4} & 
%  \midpointgradientcell{-9.7}{-4.6}{4.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-7.5}{1.8}{0}{neg}{pos}{\opacity}{0} & 

%  \baseline{2.1} & 
%  \midpointgradientcell{20.8}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}&
 
%  %qasper
%   \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0}

%     \baseline{} & 
%   \midpointgradientcell{}{-8.9}{22.8}{0}{neg}{pos}{\opacity}{0} & 
%   \midpointgradientcell{}{-8.3}{10.9}{0}{neg}{pos}{\opacity}{0} \\

\bottomrule
\end{tabular}}
\caption{Results for the abstention ability across different models for \textbf{answerable questions} 
 and \textbf{unanswerable questions} in various datasets. \textit{We find providing random context to \bioasq dataset makes all models fail to abstain.}
 \textit{RC} for random context. Colors indicate a \hlpos{positive} or \hlneg{negative} delta from the \hlbase{base score with given context}. Notice that models with higher base scores are better at abstaining.}  
\label{tab:random_context}
\end{table*}

==> tables/squad_context.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|ccccc|ccccc|ccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c|}{\textbf{ChatGPT}} & \multicolumn{5}{c|}{\textbf{\gpt}} & \multicolumn{5}{c|}{\textbf{LLamaV2}}  \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen &\scriptsize Given  & \scriptsize +Giv & \scriptsize +Rand & \scriptsize +Wiki  & \scriptsize +Gen & \scriptsize Given  & \scriptsize +Giv & \scriptsize +Rand & \scriptsize +Wiki  &  \scriptsize +Gen \\
\midrule
\parbox[t]{1mm}{\multirow{3}{*}} 
 \scriptsize All & 
 %chatgpt
 \baseline{56.1} & 
 \midpointgradientcell{65.2}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{61.1}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 


%gpt3
 \baseline{85.6} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&

%llama
 \baseline{40.0} & 
 \midpointgradientcell{1.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}

 \\

 
 \scriptsize None& 
 \baseline{97.1} & 
 \midpointgradientcell{96.8}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{88.4}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{100}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}& \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&


 \baseline{85.6} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&

%llama
 \baseline{22.7} & 
 \midpointgradientcell{0.9}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{5.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}
   \\

 \scriptsize Ext. & 
 %chatgpt
 \baseline{56.1} & 
 \midpointgradientcell{65.2}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{61.1}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&


%gpt3
 \baseline{85.6} & 
 \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&


%llama
 \baseline{57.3} & 
 \midpointgradientcell{1.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}
 
 \\


\bottomrule
\end{tabular}}
\caption{Results for the F1 performance across different models and various question types on \squad dataset. }
\label{tab:pubmed}
\end{table*}




==> tables/squad_context_new.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{\linewidth}{!}{\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c|}{\textbf{\llama}}& \multicolumn{3}{c|}{\textbf{\vicuna}}& \multicolumn{3}{c|}{\textbf{\flan}}& \multicolumn{3}{c|}{\textbf{\chatgpt}}    \\
\scriptsize\textbf{Q Type} & 
\scriptsize Given & \scriptsize +Giv & \scriptsize +Rand &\scriptsize Given  & \scriptsize +Giv & \scriptsize +Rand  & \scriptsize Given  & \scriptsize +Giv & \scriptsize +Rand  & \scriptsize Given  & \scriptsize +Giv & \scriptsize +Rand \\
\midrule
\parbox[t]{1mm}{\multirow{3}{*}} 
 \scriptsize All & 

%llama
 \baseline{40.0} & 
 \midpointgradientcell{1.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{0.4}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 %  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}

%vicuna
 \baseline{42.6} & 
 \midpointgradientcell{-1.4}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-6.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &

 %flan
 \baseline{82.6} & 
 \midpointgradientcell{-18.6}{-16.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-10.9}{-15.5}{4.1}{0}{neg}{pos}{\opacity}{0} &




 
 %chatgpt
 \baseline{64.5} & 
 \midpointgradientcell{-0.7}{-6.1}{66.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-3.4}{-6.1}{64.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 %  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 


% %gpt3
%  \baseline{85.6} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
%  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&



 \\

 
 \scriptsize None& 

%llama
 \baseline{22.7} & 
 \midpointgradientcell{0.9}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{5.1}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 
 
 % \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}


%vicuna
 \baseline{36.1} & 
 \midpointgradientcell{-5.0}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-7.6}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} & 

 %flan
 \baseline{80.6} & 
 \midpointgradientcell{-18.5}{-16.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-0.8}{-15.5}{14.1}{0}{neg}{pos}{\opacity}{0} & 

 
 %chatgpt
 \baseline{39.5} & 
 \midpointgradientcell{1.7}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-0.8}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{100}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}& \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&

% %gpt3
%  \baseline{85.6} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
%  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&

   \\

 \scriptsize Ext. & 

 %llama
 \baseline{57.3} & 
 \midpointgradientcell{1.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &
 %  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 % \midpointgradientcell{}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0}


%llama
 \baseline{57.3} & 
 \midpointgradientcell{1.1}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-4.3}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} &


%flan
 \baseline{84.5} & 
 \midpointgradientcell{-18.8}{-16.1}{16.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-20.9}{-15.5}{14.1}{0}{neg}{pos}{\opacity}{0} &
 
 %chatgpt
 \baseline{77.6} & 
 \midpointgradientcell{-3.2}{-6.1}{6.7}{0}{neg}{pos}{\opacity}{0} &
 \midpointgradientcell{-6.0}{-5.5}{4.1}{0}{neg}{pos}{\opacity}{0} 
 % \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&
 %  \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&


% %gpt3
%  \baseline{85.6} & 
%  \midpointgradientcell{}{-6.1}{76.7}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0} &
%  \midpointgradientcell{96.2}{-5.5}{74.1}{0}{neg}{pos}{\opacity}{0}&
%   \midpointgradientcell{55.5}{-5.5}{64.1}{0}{neg}{pos}{\opacity}{0}&



 
 \\


\bottomrule
\end{tabular}}
\caption{Results for the F1 performance across different models and various question types on \squad dataset. }
\label{tab:squad_context_new}
\end{table*}



